Risk-Aware Submodular Optimization for Multi-objective Travelling Salesperson Problem

We introduce a risk-aware multi-objective Traveling Salesperson Problem (TSP) variant, where the robot tour cost and tour reward have to be optimized simultaneously. The robot obtains reward along the edges in the graph. We study the case where the rewards and the costs exhibit diminishing marginal gains, i.e., are submodular. Unlike prior work, we focus on the scenario where the costs and the rewards are uncertain and seek to maximize the Conditional-Value-at-Risk (CVaR) metric of the submodular function. We propose a risk-aware greedy algorithm (RAGA) to find a bounded-approximation algorithm. The approximation algorithm runs in polynomial time and is within a constant factor of the optimal and an additive term that depends on the optimal solution. We use the submodular function's curvature to improve approximation results further and verify the algorithm's performance through simulations.

==> Risk Aware TSP/algorithmAnalysis.tex <==
\section{Algorithm And Analysis}\label{sec: algo_&_analysis}


In this section, we present a risk-aware greedy algorithm (\texttt{RAGA}) that extends the deterministic algorithm in \cite{jawaid2013maximum} for solving Problem~\ref{prob:risk-tsp}. We first  introduce \texttt{RAGA}, then analyze its performance  and running efficiency.  
\subsection{Algorithm}
\texttt{RAGA} has three main stages:\newline
%\begin{itemize}
    %\item 
    \noindent \textbf{(i) Initialization} (lines \ref{line:init} - \ref{line:init_tau})
    The decision set $\mathcal{S}$ (Hamiltonian cycle) is initialized as an empty set. A degree vector $D$ is set as $\mathbf{0}_{1 \times |\mathcal{V}|}$, which contains vertices' degrees in order. We use  variables $\hat{H}_{\text{max}}=0$ and $\hat{H}_{\text{cur}}=0$ store the maximal and the current values of $\hat{H}(\mathcal{S}, \tau)$ (line \ref{line:init}). \newline
    \noindent \textbf{(ii) Search for valid tour for every $\tau$} (lines \ref{line:while_start} - \ref{line:while_end}): For a specific value of $\tau$, we continue to add edges greedily until we have a complete tour or the edge set $\mathcal{E}$ is empty. For every edge $e \in \mathcal{E} \setminus \mathcal{S}$, we calculate the marginal gain of the auxiliary function, $\hat{H}(\mathcal{S} \cup \{e\}) - \hat{H}(\mathcal{S})$ using the oracle function $\mathbb{O}$, and choose the edge $e^{*}$ which maximizes the marginal gain (line \ref{line:oracle}). We then check if the selected edge $e^{*}$ forms (or could form) a valid tour with the elements in $\mathcal{S}$ (i.e., if $\mathcal{S} \cup \{e^{*}\} \in \mathcal{I}$) (lines \ref{line:check_start} - \ref{line:check_end}). Here, we first validate the degree constraint for each edge in $\mathcal{S} \cup \{e\}$, and then use the depth-first search (DFS) algorithm to iterate through the selected edges to check for subtours. %\footnote{A Hamiltonian cycle does not allow the existence of any subtour.}.
    If the new edge does not break the above constraints, then we add the edge in $\mathcal{S}$ and update $D$ and $\hat{H}_{cur}$ (lines \ref{line:add_edge_start} - \ref{line:add_edge_end}). Finally, we remove $e^{*}$ from $\mathcal{E}$ in line \ref{line:remove_e}.\newline 
    %\item
    \noindent \textbf{(iii) Selecting best tour set ($\mathcal{S}^{G}, \tau^{G}$)} (lines \ref{line:best_tour_start} - \ref{line:best_tour_end}): For every tour we store the value of the auxiliary function $\hat{H}$ in $\hat{H}_{\text{cur}}$, and compare it to the best value $\hat{H}_{\text{max}}$. We  store the pair $(\mathcal{S}, \tau)$ whenever $\hat{H}_{\text{cur}}> \hat{H}_{\text{max}}$, and update $\hat{H}_{\text{max}}$. 


Line 21 shows the condition of exiting the loop. As $H(\mathcal{S}, \tau)$ is concave in $\tau$, and we start from a non-negative value (as seen in Fig. \ref{fig:H_vs_tau}), it is certain that if $H(\mathcal{S}, \tau)$ becomes negative, it will continue to further decrease. This improves the runtime of \texttt{RAGA}.

\noindent \textbf{Designing the oracle function $\mathbb{O}$}: We use a sampling based oracle function to approximate $H(\mathcal{S}, \tau)$ as $\hat{H}(\mathcal{S}, \tau)$. In  \cite{ohsaka2017portfolio}, it is  proved that if the number of samples $n_{s} = O(\frac{\Gamma^{2}}{\epsilon^{2}}\log\frac{1}{\delta})$, $\delta, \epsilon \in (0,1)$, the approximation for the value of CVaR (or equivalently, the auxiliary function $\hat{H}(\mathcal{S}, \tau)$) gives an error less than $\epsilon$ with a probability of at least $1-\delta$.

\begin{algorithm}
\SetAlgoLined
\nonl \textbf{Input}: ~$G(\mathcal{V,E})$;  $\alpha \in (0,1]$; $\beta \in [0,1]$; $\Gamma \in \mathbb{R}^+$ on $\tau$; $\gamma \in (0, \Gamma]$; Oracle function $\mathbb{O}$.\\%that approximates $H(\mathcal{S}, \tau)$ as $\hat{H}(\mathcal{S}, \tau)$. \\
\nonl \textbf{Output}:  Hamiltonian tour $S^{G}$ and its respective $\tau^{G}$.\\
\For {i = \{0, 1, 2, . . ., $\ceil*{\frac{\Gamma}{\gamma}}$\}}{\label{line:for_start}
  $\mathcal{S} = \emptyset$; $D = \mathbf{0}_{1 \times |\mathcal{V}|}$; \label{line:init} $\hat{H}_{\text{max}} = 0$; $\hat{H}_{\text{cur}} = 0$, $\tau_{i} = i\,\gamma$ \\ \label{line:init_tau}
  \While {\label{line:while_start} $\mathcal{E} \neq \emptyset$ \textbf{and} $\mathcal{|S|} \leq |\mathcal{V}|$} {
    $e^\star = \text{argmax}_{{\forall e \in \mathcal{E} \setminus \mathcal{S}}} \; \hat{H}(\mathcal{S} \cup \{e\}, \tau_{i}) - \hat{H}(\mathcal{S}, \tau_{i})$\label{line:oracle}  \\ %\text{argmax}_{\forall e \in \mathcal{E} \setminus \mathcal{S}}
    $(u, v) \leftarrow \mathcal{V}(e^\star)$, $\text{flag} = \texttt{False}$\\
    \If {$D[u]<2$ \textbf{and} $D[v]<2$}{\label{line:check_start}
        check subtour existence in $\mathcal{S}\cup \{e^{\star}\}$ by running DFS\label{line:DFS}\\
        {\bf if} {\textit{no subtour present}}{~\bf then~}{ $\text{flag} = \texttt{True}$        }
    }\label{line:check_end}
    \If {$\text{flag} == \texttt{True}$}{\label{line:add_edge_start}
        $\mathcal{S} \leftarrow \mathcal{S} \cup \{e^\star\}$ \label{line:update}; $D[u] += 1$; $D[v] += 1$\\
        $\hat{H}_{\text{cur}} = \hat{H}(\mathcal{S} \cup \{e^\star\}, \tau_{i})$
   } \label{line:add_edge_end}
   $\mathcal{E} \leftarrow \mathcal{E} \setminus \{e^\star\}$ \label{line:remove_e}
  }\label{line:while_end}
  \If {$\hat{H}_{\text{cur}} \geq \hat{H}_{\text{max}}$}{\label{line:best_tour_start}
    $\hat{H}_{\text{max}} = \hat{H}_{\text{cur}}$; $(\mathcal{S}^{G}, \tau^{G})  = (\mathcal{S}, \tau_{i})$
  }\label{line:best_tour_end}
  {\bf if} {\it $\hat{H}_{\text{cur}} < 0$}~{\bf then break}\\
} \label{line:for_end}
 \caption{Risk-aware greedy algorithm (\texttt{RAGA})} \label{alg:riskg}
\end{algorithm}





\subsection{Performance Analysis}

\begin{theorem}
Let $\mathcal{S}^{G}$ and $\tau^G$ be the tour and the searching scalar selected by \texttt{RAGA} and let $\mathcal{S}^{\star}$ and $\tau^{\star}$ be the tour and the searching scalar selected the optimal solution. Then,
\begin{equation}
    H(\mathcal{S}^{G}, \tau^G)  \geq \frac{1}{2+\mathit{k}}(H(\mathcal{S}^{\star}, \tau^\star)-\gamma) + \frac{1+\mathit{k}}{2+\mathit{k}}\Gamma(1 - \frac{1}{\alpha}) - \epsilon
        \label{eqn:appro_bound}
\end{equation}
with a probability of at least $1-\delta$, when the number of samples $n_{s} = O(\frac{\Gamma^{2}}{\epsilon^{2}}\log\frac{1}{\delta}), \; \delta, \epsilon \in (0,1)$. $k$ is the curvature of $H(\mathcal{S}, \tau)$ with respect to $\mathcal{S}$.
\label{thm:approximation}
\end{theorem}

%\begin{proof}
\proof Note that $H(\mathcal{S}, \tau)$ is monotone increasing, submodular, but not normalized (Lemma \ref{lemma:properties}).  \cite[Theorem 6.1]{conforti1984submodular} and \cite[Theorem 2.10]{jawaid2013maximum} have shown that for a normalized submodular increasing function, the greedy algorithm gives an approximation of $\frac{1}{2+\mathit{k}}$ for maximizing it. Following this result, normalizing $H(\mathcal{S}, \tau)$ by $H(\mathcal{S}, \tau)-H(\emptyset, \tau)$, we get:
\begin{equation}
    \frac{H(\mathcal{S}^{G}, \tau) - H(\emptyset, \tau)}{H(\mathcal{S}^{\star}, \tau) - H(\emptyset, \tau)} \geq \frac{1}{2+\mathit{k}}
\end{equation}
where $H(\mathcal{S}^{\star}, \tau)$ is the optimal value of $H(\mathcal{S}, \tau)$ for any given value of $\tau$. Then following the proof of Theorem 1 in  \cite{zhou2020risk}, we have the bound approximation performance of \texttt{RAGA} in Equation~(\ref{eqn:appro_bound}).  $\hfill \Box$


\begin{theorem}
\texttt{RAGA} has a polynomial running time of $O(\lceil \frac{\Gamma}{\gamma} \rceil(|\mathcal{V}|^{3} (\mathcal{|V|}n_{p}+n_{s} + 2 \log |\mathcal{V}| + 1)))$.
\label{thm:complexity}
\end{theorem} 

%\begin{proof}
\proof First, the outer \textit{``for"} loop  (lines \ref{line:for_start}-\ref{line:for_end}) takes at most $\lceil \frac{\Gamma}{\gamma} \rceil$ time to search for $\tau$. Second, the inner \textit{``while"} loop (lines \ref{line:while_start}-\ref{line:while_end}) needs to check for edges $e \in \mathcal{E}$ to find the tour $\mathcal{S}$, thus running at most $|\mathcal{E}|$ times. 

Within the \textit{``while"} loop, \texttt{RAGA} finds the edge $e^{\star}$ with maximal marginal gain in line \ref{line:oracle}. To compute the marginal gain for an edge $e$, \texttt{RAGA} calls the oracle function $\mathbb{O}$. As it estimates $\hat{H}(\mathcal{S}, \tau_{i}), \forall e \in \mathcal{E} \setminus \mathcal{S}$, $\mathbb{O}$ is called at most $\mathcal{|E|}$ times, during one iteration of the \textit{``while"} loop in line \ref{line:while_start}. As \texttt{RAGA} needs to compute the marginal gains only when $\mathcal{S}$ is changed in line \ref{line:update}, and as $\mathcal{S}$ can have only $\mathcal{|V|}$ elements, it needs to perform a total of $|\mathcal{V}|$ recalculations. In addition, the edges need to be sorted every time a recalculation is performed, so that future calls to find the most beneficial element can be run in constant time without recomputing $\hat{H}(\mathcal{S}, \tau_{i})$.

For any edge $e$, the oracle $\mathbb{O}$ must compute the new mean reward and cost of $\mathcal{S} \cup \{e\}$. As only the distinct points in the environment are considered while calculating reward, the oracle must maintain an array of points that were observed while traveling along $\mathcal{S}$. If the maximum points observed when traveling along any edge in $\mathcal{E}$ is $n_{p}$, then the maximum number of points observed while traversing $\mathcal{S}$ would be $|\mathcal{V}|n_{p}$. Afterward, the oracle takes $n_{s}$ samples to compute $\hat{H}(\mathcal{S}, y)$. Thus the total runtime of the oracle is $\mathcal{|V|}n_{p}+n_{s}$. Therefore, the total time for computing gains and sorting would be $O(|\mathcal{V}|(|\mathcal{E}|(\mathcal{|V|}n_{p}+n_{s}) + |\mathcal{E}| \log |\mathcal{E}|))$.

Next, within the \textit{``while"} loop, \texttt{RAGA} checks if a the selected edge $e^{*}$ could form a valid tour with $\mathcal{S}$ (lines \ref{line:check_start}-\ref{line:check_end}). In particular, it ensures the degree of the two vertices of edge $e^\star$ is less than two (line \ref{line:check_start}). If both vertices have a degree less than two, it runs DFS to traverse the elements in $\mathcal{S}$ to check for subtours (line \ref{line:DFS}), which takes at most $|\mathcal{V}|$ time. As this is performed for every edge $e$ to be added to $\mathcal{S}$, in total, validating the selected edge runs in $O(|\mathcal{V}||\mathcal{E}|)$ time. 

Assuming that all other commands take constant time, \texttt{RAGA} has a runtime of $O(|\mathcal{V}|(|\mathcal{E}|(\mathcal{|V|}n_{p}+n_{s}) + |\mathcal{E}| \log |\mathcal{E}|) + |\mathcal{V}||\mathcal{E}|)$ for one iteration of the \textit{``for"} loop. Notably, for a complete graph, $|\mathcal{E}| = O(|\mathcal{V}|^{2})$. Considering that the \textit{``for"} loop has $\lceil \frac{\Gamma}{\gamma} \rceil$ iterations, the total runtime of \texttt{RAGA} becomes $O(\lceil \frac{\Gamma}{\gamma} \rceil(|\mathcal{V}|^{3} (\mathcal{|V|}n_{p}+n_{s} + 2 \log |\mathcal{V}| + 1)))$. $\hfill \Box$



\begin{table*}\tiny
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule 
% Group $\rightarrow$    & \multicolumn{4}{|@{}c@{\hskip0.25in}|}{Group 1} & \multicolumn{4}{@{}c@{\hskip0.25in}|}{Group 2}  & \multicolumn{3}{@{}c@{\hskip0.25in}}{Group 3} \\ 
% \midrule
\diagbox[width=3em]{\boldmath$\alpha$}{\boldmath$\beta$}  & \rotatebox[origin=c]{0}{\boldmath$0$}  & \rotatebox[origin=c]{0}{\boldmath$0.1$}  & \rotatebox[origin=c]{0}{\boldmath$0.2$}  & \rotatebox[origin=c]{0}{\boldmath$0.3$}  & \rotatebox[origin=c]{0}{\boldmath$0.4$}   & \rotatebox[origin=c]{0}{\boldmath$0.5$}  & \rotatebox[origin=c]{0}{\boldmath$0.6$}   & \rotatebox[origin=c]{0}{\boldmath$0.7$}  & \rotatebox[origin=c]{0}{\boldmath$0.8$}  & \rotatebox[origin=c]{0}{\boldmath$0.9$}  & \rotatebox[origin=c]{0}{1}  \\ \midrule
\boldmath$0.01$ & 122 \textbf{/} 145 & 121 \textbf{/} 144 & 124 \textbf{/} 141 & 126 \textbf{/} 134 & 129 \textbf{/} 136 & 127 \textbf{/} 136 & 132 \textbf{/} 138 & 127 \textbf{/} 133 & 130 \textbf{/} 131 & 132 \textbf{/} 138 & 137 \textbf{/} 135  \\
\boldmath$0.1$ & 121 \textbf{/} 149 & 122 \textbf{/} 148 & 121 \textbf{/} 149 & 125 \textbf{/} 146 & 121 \textbf{/} 145 & 136 \textbf{/} 132 & 136 \textbf{/} 137 & 135 \textbf{/} 136 & 135 \textbf{/} 133 & 130 \textbf{/} 131 & 134 \textbf{/} 131 \\ 
\boldmath$0.2$ & 124 \textbf{/} 144 & 121 \textbf{/} 143 & 124 \textbf{/} 140 & 124 \textbf{/} 147 & 134 \textbf{/} 139 & 137 \textbf{/} 139 & 144 \textbf{/} 134 & 129 \textbf{/} 138 & 138 \textbf{/} 138 & 138 \textbf{/} 130 & 134 \textbf{/} 133 \\ 
\boldmath$0.3$ & 138 \textbf{/} 137 & 127 \textbf{/} 142 & 133 \textbf{/} 133 & 135 \textbf{/} 136 & 138 \textbf{/} 138 & 138 \textbf{/} 140 & 131 \textbf{/} 144 & 140 \textbf{/} 138 & 123 \textbf{/} 144 & 127 \textbf{/} 150 & 126 \textbf{/} 141 \\
\boldmath$0.4$ & 133 \textbf{/} 138 & 142 \textbf{/} 134 & 136 \textbf{/} 135 & 129 \textbf{/} 137 & 136 \textbf{/} 139 & 138 \textbf{/} 140 & 130 \textbf{/} 141 & 139 \textbf{/} 136 & 128 \textbf{/} 147 & 127 \textbf{/} 148 & 126 \textbf{/} 147 \\ 
\boldmath$0.5$ & 141 \textbf{/} 135 & 138 \textbf{/} 135 & 144 \textbf{/} 133 & 141 \textbf{/} 138 & 142 \textbf{/} 137 & 136 \textbf{/} 139 & 138 \textbf{/} 139 & 127 \textbf{/} 148 & 138 \textbf{/} 140 & 125 \textbf{/} 147 & 129 \textbf{/} 143 \\ 
\boldmath$0.6$ & 138 \textbf{/} 131 & 141 \textbf{/} 134 & 141 \textbf{/} 134 & 142 \textbf{/} 132 & 142 \textbf{/} 137 & 134 \textbf{/} 142 & 129 \textbf{/} 142 & 134 \textbf{/} 141 & 130 \textbf{/} 144 & 124 \textbf{/} 146 & 130 \textbf{/} 146 \\
\boldmath$0.7$ & 143 \textbf{/} 133 & 138 \textbf{/} 141 & 138 \textbf{/} 138 & 139 \textbf{/} 138 & 139 \textbf{/} 138 & 137 \textbf{/} 138 & 134 \textbf{/} 141 & 131 \textbf{/} 143 & 136 \textbf{/} 140 & 129 \textbf{/} 146 & 129 \textbf{/} 147 \\ 
\boldmath$0.8$ & 143 \textbf{/} 135 & 138 \textbf{/} 137 & 141 \textbf{/} 137 & 144 \textbf{/} 133 & 142 \textbf{/} 137 & 142 \textbf{/} 137 & 141 \textbf{/} 138 & 143 \textbf{/} 135 & 129 \textbf{/} 146 & 122 \textbf{/} 148 & 126 \textbf{/} 147 \\ 
\boldmath$0.9$ & 144 \textbf{/} 133 & 139 \textbf{/} 139 & 142 \textbf{/} 135 & 144 \textbf{/} 133 & 142 \textbf{/} 137 & 140 \textbf{/} 139 & 143 \textbf{/} 136 & 128 \textbf{/} 148 & 131 \textbf{/} 146 & 121 \textbf{/} 149 & 122 \textbf{/} 150 \\
\boldmath$1$ & 143 \textbf{/} 132 & 144 \textbf{/} 132 & 144 \textbf{/} 132 & 145 \textbf{/} 134 & 145 \textbf{/} 134 & 137 \textbf{/} 137 & 134 \textbf{/} 141 & 135 \textbf{/} 139 & 121 \textbf{/} 149 & 121 \textbf{/} 149 & 128 \textbf{/} 147 \\
\bottomrule
\end{tabularx}
 \caption{\label{tab:reward_vs_cost} Variations of $f_{r}(\mathcal{S}, y)/f_{c}(\mathcal{S}, y)$ with $\alpha$ and $\beta$.}
\end{table*}



==> Risk Aware TSP/intro_new.tex <==
\section{Introduction}
%\pb {The role of CVaR is missing and the motivation is missing}
Determining an optimal tour to visit all the locations in a given set while minimizing/maximizing a metric is the classical Travelling Salesperson Problem (TSP) that finds applications in robotics, logistics, etc. However, there are several applications where the environment is dynamic and uncertain, \textcolor{black}{as a result of which classical approaches to solving the TSP are insufficient.} %that may affect the tour.
Examples include determining routes to visit active volcanic regions (where the activity has temporal variability) for obtaining scientific information (as shown in Fig. \ref{fig:Hawaii}); determining routes for a logistic delivery vehicle in dense urban regions with uncertain traffic, etc. In such scenarios, the risk due to uncertainty in the travel times and/or the rewards collected along the path needs to be considered while determining the tour. %In this paper, we address the risk--aware  multi-objective routing problem by developing a rewards--risk trade-off framework. 

%We introduce risk-aware TSP by using a specific application of persistent surveillance. Consider the scenario of monitoring the volcanoes in Hawaii, which is a dangerous task and would be better done autonomously by a robot. Fig. \ref{fig:map_Hawaii} shows a map of Hawaii, with the regions of its active volcanoes marked in red. An aerial robot monitors the volcanic situation regularly and reports the condition with an onboard camera. We depict the important points of surveillance around the volcanoes in Fig. \ref{fig:key_points}. The robot travels between these surveillance points and receives a reward based on the information gathered while traversing this tour. We do not limit the total travel time or fuel spent by the robot in this work. While traveling directly above the volcano, the robot faces a higher chance of failure but gathers more information and traverses a shorter path. Whereas, while traveling around the volcano, the robot has a lower risk but must travel a longer distance while also receiving a lower reward. Fig. \ref{fig:low_cost_low_reward} and Fig. \ref{fig:high_cost_high_reward} show the paths that could be adopted based on the risk level specified for the robot. Our objective is to find a suitable tour for a single robot while considering the risk threshold and the trade-off between path cost and reward required. We use the complete graph formed by the set of all edges between every station to select a TSP tour, which optimizes the reward-risk trade-off.


%The maximum weight Hamiltonian cycle, or the maximum TSP, is a well-researched NP-hard problem, which equivalently can be formed as a minimization problem, where tour cost is minimized. Because of its computation intensity, there have been no known polynomial-time solutions, but several approximation algorithms developed. A common method of approaching the problem is using graph theory concepts to find a minimum spanning tree. In \cite{christofides1976worst}, Christofides develops an algorithm involving searching for the shortest spanning subtree with minimum cost, which has a $\frac{3}{2}$ approximation. In \cite{fisher1979analysis}, the authors give approximation bounds on undirected graphs with non-negative weights for four simple algorithms. They go on to prove that the greedy, best neighbor and 2-interchange heuristics give a $\frac{1}{2}$ approximation, while the perfect 2-matching gives a $\frac{2}{3}$ approximation. The authors of \cite{jawaid2013maximum}, develop two approximation algorithms on a submodular cost function with an approximation factor of $\frac{1}{2+k}$ and $\max\{\frac{2}{3(2+k)}, \frac{2(1-k)}{3})\}$, where $k$ is the curvature of the function.

%Another popular idea is using Linear Programming techniques to find a solution, given certain bounds on variables. Bellman \cite{bellman1962dynamic} introduces a simple method for formulating the TSP in dynamic programming terms. Similarly, the authors in \cite{gavish1978travelling} use the Lagrangian Relaxation and sub-gradient optimization to approach the Inter Programming TSP.

%Recently, there has been a rise in evolutionary algorithms, meta-agents, and learning methods to tackle the TSP. In \cite{akhand2020discrete}, the authors use a meta-agent to find near-optimal paths. In \cite{joshi2019efficient}, the authors create a Graph Convolutional Neural Network to solve the TSP in 2D Euclidean graphs approximately. Another idea was to build a policy network that improves an initial solution by iteratively performing a neighborhood search \cite{wulearning}. 

Several approaches to stochastic TSP have been presented in the literature.  In \cite{perboli2017progressive}, a two-step process to convert the TSP to a multi-integer linear programming problem and then introduce a meta-heuristic based on the probabilistic hedging method proposed in \cite{rockafellar1991scenarios} is carried out. Paulin \cite{paulin2014convex} uses an extension of Stein's method for exchangeable pairs to approach the stochastic salesperson problem. In \cite{maity2015modified}, \cite{maity2016imprecise} and \cite{mukherjee2019constrained}, the authors develop a genetic algorithm to approach the uncertainty in TSP. In \cite{itani2007stochastic}, a constant factor approximation algorithm is developed for a Dubin's vehicle visiting all the points, with cost minimization being the main objective. In \cite{adler2016stochastic}, again an approximation algorithm is presented to minimize the time taken to visit the targets that are appearing stochastically in the environment. In all the above articles, the risk is not considered directly. 

We argue that a different approach is necessary in many risk-sensitive applications. Specifically, instead of optimizing the expected cost, optimizing a risk-sensitive measure may be more appropriate. In this paper, we focus on this case and present a risk-aware TSP formulation. To do so, we develop an approximation to the stochastic TSP with \textcolor{black}{the optimization objective} represented as a submodular function. The resulting algorithm takes as input a risk tolerance parameter, $\alpha$, and produces a tour that maximizes the expected behavior in the worst $\alpha$ percentile cases. Thus, the user can choose tours ranging from risk-neutral ($\alpha = 1$) to very conservative ($\alpha\approx 0$).

%\lz{it would be better to replace this paragraph by the work on TSP with uncertainty/stochastic tsp, then it can naturally transition to the next paragraph} \rb{addressed} \lz{exchange these 2 for a better organisation}
\begin{figure*}[t]
\begin{multicols}{4}
    \includegraphics[width=\linewidth]{figs/map_filled.eps}\subcaption{An image of an island, with the locations of active volcanoes highlighted in red}\label{fig:map_Hawaii}\par
    \includegraphics[width=\linewidth]{figs/key_points.eps}\subcaption{Key sites of surveillance surrounding the volcanic sites}\label{fig:key_points}\par
    \includegraphics[width=\linewidth]{figs/low_cost_low_reward.eps}\subcaption{Tour with low cost and low reward}\label{fig:low_cost_low_reward}\par 
    \includegraphics[width=\linewidth]{figs/high_cost_high_reward.eps}\subcaption{Tour with high cost and high reward}\label{fig:high_cost_high_reward}\par
\end{multicols}
\caption{An example of risk-aware tour selection for volcano monitoring in an island. A low-risk, low-reward monitoring tour avoids the more interesting region in the middle which the high-risk, high-reward tour covers.}\label{fig:Hawaii} 
%\lz{fig1 and 2 together}
\end{figure*}
An important property of submodular functions are their diminishing marginal values. The use of submodular functions is wide-spread: from information gathering \cite{krause2011submodularity} and image segmentation \cite{boykov2001interactive} to document summarization \cite{lin2011class}. Rockafellar and Uryasev \cite{rockafellar2000optimization} introduce a relationship between a  submodular function and the Conditional-Value-at-Risk (CVaR). CVaR is a risk metric that is commonly employed in stochastic optimization in finance and stock portfolio optimization.
%They then propose an auxiliary function by which the CVaR can be maximized. 
Another popular measure of risk is the Value-at-Risk (VaR) \cite{morgan1997creditmetrics}, which is commonly used to formulate the chance-constrained optimization problems.
In \cite{yang2017algorithm}, and \cite{yang2018algorithm}, the authors study the chance-constrained optimization problem while also considering risk in the multi-robot assignment, and then extend it to a knapsack formulation. In a comparison between the VaR and CVaR, Majumdar and Pavone \cite{majumdar2020should} propose that the CVaR is a better measure of risk for robotics, especially when the risk can cause a huge loss. In \cite{zhou2018approximation} and \cite{zhou2020risk}, a greedy algorithm for maximizing the CVaR is proposed.  

Building on the work by \cite{zhou2018approximation,zhou2020risk}, in this paper, %we leverage this prior work on choosing an unordered set to develop the first risk-aware optimization for choosing an ordered tour. {Our major contribution is the
we develop a polynomial-time algorithm for approximating a solution to the stochastic TSP. Our method differs from the previous approaches due to the presence of uncertainty in the tour cost, making traditional path-planning algorithms fail. The framework presented in \cite{zhou2018approximation,zhou2020risk} is effective only for one-stage planning (selecting a path amongst a set of candidate paths). In this paper, we present a multi-stage planner that finds a route taking the stochastic aspect into account. To achieve this, we propose an objective function that balances  risk and reward for a tour and prove that this function is submodular. %  whereas the algorithm developed in this paper finds a balance between two opposing functions formed from the rewards and costs. Our algorithm plans an entire TSP tour, which is fundamentally more challenging than selecting a path amongst a set of candidate paths for the vehicle assignment in \cite{zhou2018approximation,zhou2020risk
%We can say 15-16 were not designed for finding tours but just selecting from amongst a set of candidate paths. Here, we are *planning* for a path so the algorithm needs to take that into account. We can also say that another novel contribution is this function that balancesand showing that it is submodular.
 The method in \cite{jawaid2013maximum} addresses the deterministic TSP with a reward-cost trade-off, while our work is focused  on a stochastic version where the uncertainty in reward and cost is considered. The algorithm from \cite{jawaid2013maximum} can be viewed as a special case of our algorithm, with $\alpha=1$ and the subsequent risk ignored.
%We determine a single solution set to maximize the CVaR using a monotone submodular function \cite{zhou2018approximation}. The optimization problem is then framed over a matroid constrained system.


\noindent \textbf{Contributions}:  The main contributions of this paper are:
\begin{itemize}%Risk-Aware Multi Objective%
    \item \textcolor{black}{We present a risk-aware TSP with a stochastic objective that balances risk and reward for planing a TSP tour (Problem~\ref{prob:risk-tsp}). 
    \item We show the objective is submodular (Lemma~\ref{lemma:sub and monotone}) and }propose a greedy algorithm (\texttt{RAGA}) to find tours that maximize the CVaR of a stochastic objective (Algorithm~\ref{alg:riskg}).
    \item We prove that the solution obtained by \texttt{RAGA} is within a constant approximation factor of the optimal and an additive term proportional to the optimal solution (Theorem~\ref{thm:approximation}) and prove that \texttt{RAGA} has a polynomial run-time (Theorem~\ref{thm:complexity}). 
    \item We evaluate the performance of the algorithm through extensive simulations (Section~\ref{sec: results}).
\end{itemize}

% \indent \textbf{Organization}: The rest of the paper is organized as follows. In Sec. \ref{sec: prelim}, the necessary background materials on  sets, function properties, VaR, and CVaR is given. In Sec. \ref{sec: prob_form}, we describe risk-aware  TSP and the multi-objective optimization problem. Subsequently, we present our main algorithm \texttt{RAGA} and then derive its performance in Sec. \ref{sec: algo_&_analysis}. In Sec. \ref{sec: results}, we show simulation results of \texttt{RAGA}. Finally, in Sec. \ref{sec: conc}, we conclude and discuss future work.

==> Risk Aware TSP/intro_new1.tex <==
\section{Introduction}
%\pb {The role of CVaR is missing and the motivation is missing}
Determining an optimal tour to visit all the locations in a given set while minimizing/maximizing a metric is the classical Travelling Salesperson Problem (TSP) that finds applications in robotics, logistics, etc. However, there are several applications where the environment is dynamic and uncertain, as a result of which classical approaches to solving the TSP are insufficient.
Examples include determining routes to visit active (temporal variability) volcanic regions as shown in Fig. \ref{fig:Hawaii}. %; determining routes for a logistic delivery vehicle in dense urban regions with uncertain traffic, etc.
 In such scenarios, the risk due to uncertainty in the travel times and/or the rewards collected along the path needs to be considered while determining the tour.

Several approaches to stochastic TSP have been presented in the literature.  In \cite{perboli2017progressive}, a two-step process to convert the TSP to a multi-integer linear programming problem and then introduce a meta-heuristic based on the probabilistic hedging method proposed in \cite{rockafellar1991scenarios} is carried out. Paulin \cite{paulin2014convex} uses an extension of Stein's method for exchangeable pairs to approach the stochastic salesperson problem. In \cite{maity2015modified,maity2016imprecise,mukherjee2019constrained}, a genetic algorithm is used  to consider uncertainty in TSP. In \cite{itani2007stochastic,adler2016stochastic},  approximation algorithms are developed for the stochastic TSP with Dubin's vehicle motion constraints. %visiting all the points, with cost minimization being the main objective. In \cite{adler2016stochastic}, again an approximation algorithm is presented to minimize the time taken to visit the targets that are appearing stochastically in the environment.
 In all the above articles, the risk is not considered directly. 

We argue that a different approach is necessary in many risk-sensitive applications. Specifically, instead of optimizing the expected cost, optimizing a risk-sensitive measure may be more appropriate. In this paper, we  present a risk-aware TSP formulation. To do so, we develop an approximation to the stochastic TSP with {the optimization objective} represented as a submodular function. The resulting algorithm takes  a risk tolerance parameter $\alpha$ as input and produces a tour that maximizes the expected behavior in the worst $\alpha$ percentile cases. Thus, the user can choose tours ranging from risk-neutral ($\alpha = 1$) to very conservative ($\alpha\approx 0$).
\begin{figure*}
\begin{multicols}{5}
    \includegraphics[width=3cm,height=3.5cm]{figs/map_filled.eps}\subcaption{}\label{fig:map_Hawaii}\par
    \includegraphics[width=3cm,height=3.5cm]{figs/key_points.eps}\subcaption{}\label{fig:key_points}\par
    \includegraphics[width=3cm,height=3.5cm]{figs/high_cost_high_reward.eps}\subcaption{}\label{fig:high_cost_high_reward}\par
        \includegraphics[width=3cm,height=3.5cm]{figs/low_cost_low_reward.eps}\subcaption{}\label{fig:low_cost_low_reward}\par 
        \includegraphics[clip,trim=20mm 8mm 20mm 15mm, width=3cm,height=3.5cm]{figs/info_map.png}\subcaption{}\label{fig:info_map}\par 
\end{multicols}\vspace{-0.4cm}
\caption{An example of risk-aware tour selection for volcano monitoring in an island. (a) The areas of active volcanoes (red regions) (b) Key sites of surveillance surrounding the volcanic sites (c) Tour with high cost and high reward (d) Tour with low cost and low reward (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
\end{figure*}

%\begin{figure*}[t]
%\begin{multicols}{4}
%    \includegraphics[width=3cm,height=4cm]{figs/map_filled.eps}\subcaption{}\label{fig:map_Hawaii}\par
%    \includegraphics[width=3cm,height=4cm]{figs/key_points.eps}\subcaption{}\label{fig:key_points}\par
%    \includegraphics[width=3cm,height=4cm]{figs/high_cost_high_reward.eps}\subcaption{}\par
%        \includegraphics[width=3cm,height=4cm]{figs/low_cost_low_reward.eps}\subcaption{}\label{fig:low_cost_low_reward}\par 
%        \includegraphics[width=3cm,height=4cm]{figs/info_map.png}\subcaption{Tour with low cost and low reward}\label{fig:info_map}\par 
%\end{multicols}
%\caption{An example of risk-aware tour selection for volcano monitoring in an island. (a). An island with the locations of active volcanoes (red regions) (b) Key sites of surveillance surrounding the volcanic sites (c) Tour with high cost and high reward}\label{fig:high_cost_high_reward (d) Tour with low cost and low reward (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
%\end{figure*}
%\begin{figure*}[t]
%\begin{multicols}{4}
%    \includegraphics[width=3cm,height=4cm]{figs/map_filled.eps}\subcaption{An island with the locations of active volcanoes (red regions)}\label{fig:map_Hawaii}\par
%    \includegraphics[width=3cm,height=4cm]{figs/key_points.eps}\subcaption{Key sites of surveillance surrounding the volcanic sites}\label{fig:key_points}\par
%    \includegraphics[width=3cm,height=4cm]{figs/high_cost_high_reward.eps}\subcaption{Tour with high cost and high reward}\label{fig:high_cost_high_reward}\par
%        \includegraphics[width=3cm,height=4cm]{figs/low_cost_low_reward.eps}\subcaption{Tour with low cost and low reward}\label{fig:low_cost_low_reward}\par 
%        \includegraphics[width=3cm,height=4cm]{figs/info_map.png}\subcaption{Tour with low cost and low reward}\label{fig:info_map}\par 
%\end{multicols}
%\caption{An example of risk-aware tour selection for volcano monitoring in an island. A low-risk, low-reward monitoring tour avoids the more interesting region in the middle which the high-risk, high-reward tour covers. (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
%\end{figure*}
An important property of submodular functions are their diminishing marginal values. The use of submodular functions is wide-spread: from information gathering \cite{krause2011submodularity} and image segmentation \cite{boykov2001interactive} to document summarization \cite{lin2011class}. Rockafellar and Uryasev \cite{rockafellar2000optimization} introduces a relationship between a  submodular function and the Conditional-Value-at-Risk (CVaR). CVaR is a risk metric that is commonly employed in stochastic optimization in finance and stock portfolio optimization.
%They then propose an auxiliary function by which the CVaR can be maximized. 
Another popular measure of risk is the Value-at-Risk (VaR) \cite{morgan1997creditmetrics}, which is commonly used to formulate the chance-constrained optimization problems.
In \cite{yang2017algorithm}, and \cite{yang2018algorithm}, the authors study the chance-constrained optimization problem while also considering risk in the multi-robot assignment problems. In a comparison between the VaR and CVaR, Majumdar and Pavone \cite{majumdar2020should} propose that the CVaR is a better measure of risk for robotics, especially when the risk can cause a huge loss. In \cite{zhou2018approximation} and \cite{zhou2020risk}, a greedy algorithm for maximizing the CVaR is proposed.  

Building on the work by \cite{zhou2018approximation,zhou2020risk}, in this paper, %we leverage this prior work on choosing an unordered set to develop the first risk-aware optimization for choosing an ordered tour. {Our major contribution is the
we develop a polynomial-time algorithm for approximating a solution to the stochastic TSP. Our method differs from the previous approaches due to the presence of uncertainty in the tour cost, making traditional path-planning algorithms fail. The framework presented in \cite{zhou2018approximation,zhou2020risk} is effective only for one-stage planning (selecting a path amongst a set of candidate paths). In this paper, we present a multi-stage planner that finds a route taking the stochastic aspect into account. To achieve this, we propose an objective function that balances  risk and reward for a tour and prove that this function is submodular. %  whereas the algorithm developed in this paper finds a balance between two opposing functions formed from the rewards and costs. Our algorithm plans an entire TSP tour, which is fundamentally more challenging than selecting a path amongst a set of candidate paths for the vehicle assignment in \cite{zhou2018approximation,zhou2020risk
%We can say 15-16 were not designed for finding tours but just selecting from amongst a set of candidate paths. Here, we are *planning* for a path so the algorithm needs to take that into account. We can also say that another novel contribution is this function that balancesand showing that it is submodular.
 The method in \cite{jawaid2013maximum} addresses the deterministic TSP with a reward-cost trade-off, while our work is focused  on a stochastic version where the uncertainty in reward and cost is considered. The algorithm from \cite{jawaid2013maximum} can be viewed as a special case of our algorithm, with $\alpha=1$ and the subsequent risk ignored.
%We determine a single solution set to maximize the CVaR using a monotone submodular function \cite{zhou2018approximation}. The optimization problem is then framed over a matroid constrained system.


\noindent \textbf{Contributions}:  The main contributions of this paper are:
\begin{itemize}[leftmargin=*]%Risk-Aware Multi Objective%
    \item \textcolor{black}{We present a risk-aware TSP with a stochastic objective that balances risk and reward for planning a TSP tour (Problem~\ref{prob:risk-tsp}). 
    \item We show the objective is submodular (Lemma~\ref{lemma:sub and monotone}) and }propose a greedy algorithm (\texttt{RAGA}) to find tours that maximize the CVaR of a stochastic objective (Algorithm~\ref{alg:riskg}).
    \item We prove that the solution obtained by \texttt{RAGA} is within a constant approximation factor of the optimal and an additive term proportional to the optimal solution (Theorem~\ref{thm:approximation}) and prove that \texttt{RAGA} has a polynomial run-time (Theorem~\ref{thm:complexity}). 
    \item We evaluate the performance of the algorithm through extensive simulations (Section~\ref{sec: results}).
\end{itemize}

% \indent \textbf{Organization}: The rest of the paper is organized as follows. In Sec. \ref{sec: prelim}, the necessary background materials on  sets, function properties, VaR, and CVaR is given. In Sec. \ref{sec: prob_form}, we describe risk-aware  TSP and the multi-objective optimization problem. Subsequently, we present our main algorithm \texttt{RAGA} and then derive its performance in Sec. \ref{sec: algo_&_analysis}. In Sec. \ref{sec: results}, we show simulation results of \texttt{RAGA}. Finally, in Sec. \ref{sec: conc}, we conclude and discuss future work.

==> Risk Aware TSP/intro_old.tex <==
\section{Introduction}

%\pb {The role of CVaR is missing and the motivation is missing}

The maximum weight Hamiltonian cycle (max-TSP), is a well-researched NP-hard problem, which can also be formed as a minimization problem, where tour cost is minimized. Because of its computation intensity, there have been no known polynomial-time solutions but several approximation algorithms. A common method of approaching the problem is using graph theory concepts to find a minimum spanning tree. In \cite{christofides1976worst}, Christofides develops an algorithm to search for the shortest spanning subtree with minimum cost, which has a $\frac{3}{2}$ approximation. In \cite{fisher1979analysis}, the authors give approximation bounds on undirected graphs with non-negative weights. They go on to prove that the greedy, best neighbor and 2-interchange heuristics give a $\frac{1}{2}$ approximation, while the perfect 2-matching gives a $\frac{2}{3}$ approximation. The authors of \cite{jawaid2013maximum}, develop two approximation algorithms on a submodular cost function with an approximation factor of $\frac{1}{2+k}$ and $\max\{\frac{2}{3(2+k)}, \frac{2(1-k)}{3})\}$, where $k$ is the curvature of the function.

Another popular idea is using Linear Programming techniques to find a solution, given certain bounds on the variables. Bellman \cite{bellman1962dynamic} introduces a simple method for formulating the TSP in dynamic programming terms. Similarly, the authors in \cite{gavish1978travelling} use the Lagrangian Relaxation and sub-gradient optimization to approach the Inter Programming TSP.

Recently, there has been a rise in evolutionary algorithms, meta-agents, and learning methods to tackle the TSP. In \cite{akhand2020discrete}, the authors use a meta-agent to find near-optimal paths. In \cite{joshi2019efficient}, the authors create a Graph Convolutional Neural Network to solve the TSP approximately. Another idea was to build a policy network that improves an initial solution by iteratively performing a neighborhood search \cite{wulearning}. 

The problem complexity increases when the uncertainty in tour quality is also considered. In \cite{perboli2017progressive}, the authors use a two-step process to convert the TSP to a multi-integer linear programming problem and then introduce a meta-heuristic based on the probabilistic hedging method proposed in \cite{rockafellar1991scenarios}. Paulin \cite{paulin2014convex} uses an extension of Stein's method for exchangeable pairs to approach the stochastic salesman problem. In \cite{maity2015modified}, \cite{maity2016imprecise} and \cite{mukherjee2019constrained}, the authors develop a genetic algorithm to approach the uncertainty in TSP. In this paper, we take a graph-based approach to generate an approximation to the stochastic TSP by using a submodular function. 
%\lz{it would be better to replace this paragraph by the work on TSP with uncertainty/stochastic tsp, then it can naturally transition to the next paragraph} \rb{addressed} \lz{exchange these 2 for a better organisation}


\begin{figure*}[t]
\begin{multicols}{4}
    \includegraphics[width=\linewidth]{figs/map_filled.eps}\subcaption{A map of Hawaii, with the locations of active volcanoes highlighted in red}\label{fig:map_Hawaii}\par
    \includegraphics[width=\linewidth]{figs/key_points.eps}\subcaption{Key points of surveillance surrounding the volcanic sites}\label{fig:key_points}\par
    \includegraphics[width=\linewidth]{figs/low_cost_low_reward.eps}\subcaption{Path with low cost and low reward}\label{fig:low_cost_low_reward}\par 
    \includegraphics[width=\linewidth]{figs/high_cost_high_reward.eps}\subcaption{Path with high cost and high reward}\label{fig:high_cost_high_reward}\par
\end{multicols}
\caption{An example of site placement and risk-aware path selection for volcano surveillance in Hawaii.}\label{fig:Hawaii} 
%\lz{fig1 and 2 together}
\end{figure*}

An important property of submodular functions is its diminishing marginal values. The use of submodular functions is wide-spread: from information gathering \cite{krause2011submodularity} and image segmentation \cite{boykov2001interactive} to document summarization \cite{lin2011class}. Rockafellar and Uryasev introduce a relationship between a monotone increasing, normalized, submodular function, and the Conditional-Value-at-Risk (CVaR) \cite{rockafellar2000optimization}, and propose an auxiliary function by which the CVaR can be maximized. Another measure of risk is the Value-at-Risk (VaR)\cite{morgan1997creditmetrics}, which is commonly used to formulate the chance-constrained optimization problems. In \cite{yang2017algorithm}, and \cite{yang2018algorithm}, the authors study the chance-constrained optimization problem while also considering risk in multi-robot assignment, and then extend it to a knapsack formulation. In a comparison between the VaR and CVaR, Majumdar and Pavone argue that the CVaR is a better measure of risk for robotics based on six axioms \cite{majumdar2020should}. Finally, in \cite{zhou2018approximation} and \cite{zhou2020risk}, the authors demonstrate a greedy algorithm for maximizing the CVaR.  

\indent \textbf{Contributions}: We focus on selecting a single solution set, similar to \cite{zhou2018approximation}, to maximize the CVaR using a monotone submodular function. The optimization problem is then framed over a matroid constrained system. Our contributions are as follows:

\begin{itemize}%Risk-Aware Multi Objective%
    \item We propose the Risk Aware Greedy Algorithm (\texttt{RAGA}) to select tours for the Travelling Salesman Problem that maximize the value of CVaR.
    \item We then prove that the solution found is within a constant approximation factor of the optimal set added with an additive term proportional to the optimal solution. Next, we prove that the proposed algorithm has a polynomial runtime. 
    \item We finally test the performance of the algorithm through simulations.
\end{itemize}

\indent \textbf{Organization}: The rest of the paper is organized as follows. In Sec. \ref{sec: prelim}, we discuss the necessary background material on graphs, sets, and function properties. We then formally define the concepts of VaR and CVaR. Next, in Sec. \ref{sec: prob_form}, we describe the setting of the TSP and the multi-objective optimization. Subsequently, we present the Risk Aware Greedy algorithm and then derive its performance in Sec. \ref{sec: algo_&_analysis}. In Sec. \ref{sec: results}, we show simulation results of the algorithm. Finally, in Sec. \ref{sec: conc}, we conclude and discuss the work remaining.

% \indent \textbf{Related work.}\\

%  \lz{\begin{itemize}
%   \item introduce our risk-aware TSP (refer to my WAFR paper.)
%     \item Related work, part 1: TSP, stochastic TSP using expectation, mean-variance measure, chance constraint etc. (need some search)
%     \item Related work, part 2: VaR and CVaR for robot planning. (refer to my WAFR paper.)
%     \item our contributions, 1: formulate risk-aware TSP; 2:approximation bound and polynomial running time; 3: simulation results. (Refer to my IROS paper) 
%  \end{itemize}}

==> Risk Aware TSP/prelim.tex <==
\section{Preliminaries}\label{sec: prelim}
We first introduce the conventions and notations used in this paper. Calligraphic capital letters denote sets (e.g. $\mathcal{A}$). $2^{\mathcal{A}}$ denotes the power set of $\mathcal{A}$ and $|\mathcal{A}|$ represents its cardinality. Given a set $\mathcal{B}$, $\mathcal{A \setminus B}$ denotes set difference. Let $x$ be a random variable, then $\mathbb{E}[x]$ represents the expectation of the random variable $x$, and $\mathbb{P[\cdot]}$ denotes its probability. 

\subsection{Set and Function Properties}
Optimization problems generally work over a set system $(\mathcal{X, Y})$ where $\mathcal{X}$ is the base set and $\mathcal{Y} \subseteq 2^{\mathcal{X}}$. A reward/cost function $f : \mathcal{Y} \rightarrow \mathbb{R}$ is then either maximized or minimized. 

\begin{definition}
\label{def:inc}
(Monotonically Increasing):  A set function $f : \mathcal{Y} \rightarrow \mathbb{R}$ is said to be monotonically increasing if and only if for any set $\mathcal{S'} \subseteq \mathcal{S} \in 2^{\mathcal{X}}, ~f(\mathcal{S'}) < f(\mathcal{S})$.
\end{definition}
\begin{definition}
\label{def:sub}
(Submodularity): A function $f:2^{\mathcal{X}} \rightarrow \mathbb{R}$ is submodular if and only if,
$f(\mathcal{S}) + f(\mathcal{T}) \geq f(\mathcal{S} \cup \mathcal{T}) + f(\mathcal{S} \cap \mathcal{T}), ~\forall \mathcal{S},~\mathcal{T}~\in~2^{\mathcal{X}}$.

\end{definition}
\begin{definition}
(Matroid): An independence set system $\mathcal{(X,Y)}$ is called a matroid if for any sets $\mathcal{S, P} \in 2^{\mathcal{X}}$ and $|\mathcal{P}| \leq |\mathcal{S}|$, it must hold that there exists an element $s \in \mathcal{S} \setminus \mathcal{P}$ such that $\mathcal{P} \cup \{s\} \in \mathcal{Y}$.
\end{definition}

\begin{definition}
(Curvature): Curvature is used as a measure of the degree of submodularity of a function $f$. Consider the matroid pair $(\mathcal{X, Y})$, and a function $f: 2^{\mathcal{X}} \rightarrow \mathbb{R}$, such that for any element $s \in \mathcal{X}, f(\{s\}) \neq 0$. The curvature $k,0 \leq k \leq 1$ is then defined as:
\begin{equation}\small
    k = 1 - \min_{s \in \mathcal{S}, \mathcal{S} \in \mathcal{Y}} \: \frac{f(\mathcal{S}) - f(\mathcal{S}\setminus \{s\})}{f(\{s\})}.
\end{equation}
\end{definition}\vspace{-0.3cm}

\subsection{Travelling Salesperson Problem}

\begin{definition}
(TSP): Given a complete graph $G(\mathcal{V, E})$, the objective of the TSP is to find a minimum cost (maximum reward) Hamiltonian cycle. 
\end{definition}
In this paper, we consider the symmetric undirected TSP, where each edge has a reward and cost associated with it. \vspace{-0.3cm}




\subsection{Measure of Risk}
Let $f(\mathcal{S}, y)$ denote a utility function with solution set $\mathcal{S}$ and noise $y$. As a result of $y$, the value of $f(\mathcal{S},y)$ is a random variable for every $\mathcal{S}$. 
\begin{definition}
    (Value at Risk): The Value at Risk (VaR) is defined as:
\begin{equation}
    \emph{VaR}_{\alpha}(\mathcal{S}) = \min_{\tau \in \mathbb{R}} \; \{\mathbb{P}[f(\mathcal{S}, y) \leq \tau] \geq \alpha \}, \; \alpha \in (0,1],
\end{equation}
\textcolor{black}{where $\alpha$ is the user-defined risk-level. A higher value of $\alpha$ corresponds to the choice of a higher risk level}.
\end{definition}

\begin{definition}
    (Conditional Value at Risk): The Conditional-Value-at-Risk (CVaR) is defined as
\begin{equation}
    \emph{CVaR}_{\alpha}(\mathcal{S}) = \mathbb{E}_{y} [f(\mathcal{S},y) \:|\: f(\mathcal{S},y) \leq \emph{VaR}_{\alpha}(\mathcal{S})].
\end{equation}
Maximizing the value of $\text{CVaR}_{\alpha}(\mathcal{S})$ is equivalent to maximizing the auxiliary function $H(\mathcal{S}, \tau)$ (Theorem 2, \cite{rockafellar2000optimization}):
\begin{equation}
    H(\mathcal{S}, \tau) = \tau - \frac{1}{\alpha}\mathbb{E}_y[\: (\tau - f(\mathcal{S}, y))^{+} \:],
\end{equation}
where $[t]^{+} = t, ~\forall t \geq 0$ and $0$ when $t < 0$.
\end{definition}



\begin{lemma}
\label{lemma:properties}
\textup{(Lemma 1, \cite{zhou2018approximation})} If $f(\mathcal{S},y)$ is monotone increasing, submodular and normalized in set $\mathcal{S}$ for any realization of $y$, then the auxiliary function $H(\mathcal{S}, \tau)$ is monotone increasing and submodular but not necessarily normalized \footnote{\textcolor{black}{The function $f(\mathcal{S}, y)$ is normalized in $\mathcal{S}$ if and only if $f(\emptyset, y) = 0$.}} in set $\mathcal{S}$ for any given $\tau$.
\end{lemma} 

\begin{lemma}
\textup{(Lemma 2, \cite{zhou2018approximation})} The auxiliary function $H(\mathcal{S}, \tau)$ is concave in $\tau, \forall\: \mathcal{S}$.
\end{lemma}



==> Risk Aware TSP/probFormulation.tex <==
\section{Problem Formulation} \label{sec: prob_form}
In this section, we first discuss a risk-aware TSP and then formulate the problem as a  stochastic optimization problem by using CVaR.

\subsection{Risk-Aware TSP}
In order to motivate our formulation, consider the scenario of monitoring active volcanoes using a robot (say aerial robot) on an island as shown in Fig. \ref{fig:map_Hawaii}, where the red-colored patches represent active volcanic regions.  The important sites ($\mathcal{V}$) that the robot needs to visit are shown in Fig. \ref{fig:key_points}. \textcolor{black}{These sites are strategic positions from which it is possible to observe the volcanic situation from a safe distance.} The robot travels between these monitoring sites and receives a reward based on the information gathered while traversing this tour.  While traveling directly above the volcano, the robot faces a higher chance of failure (due to volcanic activity) but can gather more information (a higher reward) and a shorter path (less cost) Fig. \ref{fig:high_cost_high_reward}. On the other hand, while traveling around the volcano, the robot has a lower risk but must travel a longer distance (more cost) while also receiving a lower reward Fig. \ref{fig:low_cost_low_reward} .  Our objective is to find a suitable tour for a single robot while considering the risk threshold and the trade-off between path cost and reward required. 

The monitoring task is modeled as a risk-aware TSP on a graph $G(\mathcal{V}, \mathcal{E})$ of an environment ${E}$ with $|\mathcal{V}|$ sites of interest and  $\mathcal{E}$ represents the set of edges connecting the vertices. A representative information density map ${M}$ of the environment ${E}$ is shown in Fig. \ref{fig:info_map}. The robot has sensors with a sensing range $R$. As it travels along the tour, the robot receives a reward based on the amount of information it collects and a penalty proportional to the tour's cost. We assume that both the reward and cost are random variables, with the reward being positive, and the cost of every edge having an upper-bound of $C$. {We use $r(\mathcal{S}, y_{r})$ and $c(\mathcal{S}, y_{c})$ to denote the reward and cost for the edge set  $\mathcal{S}$, where $r(\mathcal{S})$ and $c(\mathcal{S})$ are the sum of rewards of all points observed and the costs incurred when travelling along the edges in set $\mathcal{S}$ respectively, and  $y_{r}$ and $y_{c}$ are the respective noises induced.}


As we want to minimize cost and maximize reward simultaneously, our utility function $f(\mathcal{S},y)$ is a combination of these two terms, with a weighting factor deciding the priority of cost over the reward. We define $f(\mathcal{S},y)$ as
\begin{equation}
    f(\mathcal{S}, y) = (1-\beta)\:r(\mathcal{S}, y_{r}) +  \beta\:(|\mathcal{S}|C-c(\mathcal{S}, y_{c})),
\end{equation}
where $\beta \in [0,1]$ is the weighting parameter. When $\beta = 0$, we ignore the cost incurred and consider the rewards received only. When $\beta = 1$, we ignore the rewards and are wary of only the cost penalized (classical TSP). Note that we directly incorporate the cost-reward trade-off into the utility function. Let us define $r(\mathcal{S}, y_{r})$ as $f_{r}(\mathcal{S}, y_{r})$ and $|\mathcal{S}|C-c(\mathcal{S}, y_{c})$ as $f_{c}(\mathcal{S}, y_{c})$. 

%\begin{figure}
%    \centering
%    \includegraphics[width=6cm, height=4cm]{figs/info_map.png}
%    \caption{Map $M$ shows the information distribution in the environment $E$.} % with the density  information.}
%    \label{fig:info_map}\vspace{-0.75cm}
%\end{figure}

\begin{lemma}
The utility function $f(\mathcal{S}, y)$ is both submodular and monotone increasing in $\mathcal{S}$.
\label{lemma:sub and monotone}
\end{lemma}

%%%%%%%%%%%%%%NEW VERSION TEXT

\proof {Let $e$ be the edge to be added to the tour, where $e \in \mathcal{E} \setminus \mathcal{S}$ and $\mathcal{S}$ is set of edges selected so far. Let us consider the two parts of $f(\mathcal{S}, y)$ separately. 
 \newline {\bf (a) {$f_{r}(\mathcal{S},y)$}}: As the rewards are sampled from a truncated Gaussian, with a lower bound of 0, they are thus always positive. Therefore, $f_{r}(\mathcal{S}, y)$ is always monotone increasing in $\mathcal{S},            f_{r}(\mathcal{S}) \leq f_{r}(\mathcal{S}\cup\{e\})$.
\newline \noindent While calculating the total reward, we add the rewards obtained from all \textit{distinct} points observed while traversing this tour. Consider the current set of edges $\mathcal{S}$ and a new edge $e$. If the new edge $e$ and the edges $\mathcal{S}$ have any overlap in the sensed regions, the total reward received from traversing $\mathcal{S}$ and $e$ successively will be less than the sum of rewards of traversing $\mathcal{S}$ and $e$ individually. Therefore,
 $ f_{r}(\mathcal{S} \cup \{e\})  \leq f_{r}(\mathcal{S}) + f_{r}(\{e\})$. Also, since $e \in \mathcal{E} \setminus \mathcal{S}$, $f_{r}(\mathcal{S} \cap \{e\}) =0$. Then we have, $
            f_{r}(\mathcal{S} \cup \{e\}) + f_{r}(\mathcal{S} \cap \{e\}) \leq f_{r}(\mathcal{S}) + f_{r}(\{e\}),$ 
        and thus $f_{r}(\mathcal{S},y)$ is submodular in $\mathcal{S}$.

\noindent{\bf(b) {$f_{c}(\mathcal{S}, y)$}}: The cost of each edge is defined as a truncated Gaussian with a upper bound of $M_{c}$. For any set of edges in $\mathcal{S}$, the sum of costs will always be less than $|\mathcal{S}|M_{c}$, which means any sample (realization) of $f_{c}(\mathcal{S}, y)$ is positive. Therefore, $f_{c}(\mathcal{S}, y)$ is always monotone increasing in $\mathcal{S}$,  $ f_{c}(\mathcal{S}) \leq f_{c}(\mathcal{S}\cup\{e\}).$ Consider again, the current set of edges $\mathcal{S}$ and the new edge $e$. The total cost of traversing $\mathcal{S}$ and $e$ is equal to the sum of costs of  traversing $\mathcal{S}$ and $e$ individually. Therefore,
$            f_{c}(\mathcal{S} \cup \{e\}) = f_{c}(\mathcal{S}) + f_{c}(\{e\}), $
        and thus $f_{c}(\mathcal{S}, y)$ is modular in $\mathcal{S}$.
\newline \noindent {\bf (c) {$f(\mathcal{S}, y)$}}: Since both $f_{r}(\mathcal{S}, y_{r})$ and $f_{c}(\mathcal{S}, y_{c})$ are monotone increasing in $\mathcal{S}$, $f(\mathcal{S}, y)$ as the summation of these two, is also monotone increasing in $\mathcal{S}$. Similarly, since $f_{r}(\mathcal{S}, y_{r})$ is submodular in $\mathcal{S}$ and $f_{c}(\mathcal{S}, y_{c})$ is modular in $\mathcal{S}$, $f(\mathcal{S}, y)$ as the summation of these two, is submodular in $\mathcal{S}$.  \hfill $\Box$ 
}

\subsection{Risk-Aware  Submodular Maximization}
Consider the set system $\mathcal{(E, I)}$, where $\mathcal{E}$ is the set of all edges in the graph $G(\mathcal{V, E})$. If $\mathcal{A}_{1}, \mathcal{A}_{2} \ldots \mathcal{A}_{n}$ each contains the edges forming $n$ Hamiltonian tours, then $\mathcal{I} := 2^{\mathcal{A}_{1}} \cup 2^{\mathcal{A}_{2}} \ldots \cup 2^{\mathcal{A}_{n}}$. We define our \textit{risk-aware  TSP} by maximizing  $\text{CVaR}_{\alpha}(\mathcal{S})$, where $\mathcal{S} \in \mathcal{I}$. We know that maximizing the $\text{CVaR}_{\alpha}(\mathcal{S})$ is equivalent to maximizing the auxiliary function ${H(\mathcal{S}, \tau)}$. Thus, we formally define the problem as:

\begin{problem} [Risk-aware  TSP]
\begin{equation}
    \max_{\mathcal{S} \in \mathcal{I}, ~\tau \in [0, \Gamma]} \tau - \frac{1}{\alpha} \mathbb{E}_y[ (\tau - f(\mathcal{S}, y))^{+}], 
\end{equation}
where $\Gamma$ is the upper bound on the value of $\tau$.
\label{prob:risk-tsp}
\end{problem}



==> algorithmAnalysis.tex <==
\section{Algorithm And Analysis}\label{sec: algo_&_analysis}


In this section, we present a risk-aware greedy algorithm (\texttt{RAGA}) that extends the deterministic algorithm in \cite{jawaid2013maximum} for solving Problem~\ref{prob:risk-tsp}. We first  introduce \texttt{RAGA}, then analyze its performance  and running efficiency.  
\subsection{Algorithm}
\texttt{RAGA} has three main stages:\newline
%\begin{itemize}
    %\item 
    \noindent \textbf{(i) Initialization} (lines \ref{line:init} - \ref{line:init_tau})
    The decision set $\mathcal{S}$ (Hamiltonian cycle) is initialized as an empty set. A degree vector $D$ is set as $\mathbf{0}_{1 \times |\mathcal{V}|}$, which contains vertices' degrees in order. We use  variables $\hat{H}_{\text{max}}=0$ and $\hat{H}_{\text{cur}}=0$ store the maximal and the current values of $\hat{H}(\mathcal{S}, \tau)$ (line \ref{line:init}). \newline
    \noindent \textbf{(ii) Search for valid tour for every $\tau$} (lines \ref{line:while_start} - \ref{line:while_end}): For a specific value of $\tau$, we continue to add edges greedily until we have a complete tour or the edge set $\mathcal{E}$ is empty. For every edge $e \in \mathcal{E} \setminus \mathcal{S}$, we calculate the marginal gain of the auxiliary function, $\hat{H}(\mathcal{S} \cup \{e\}) - \hat{H}(\mathcal{S})$ using the oracle function $\mathbb{O}$, and choose the edge $e^{*}$ which maximizes the marginal gain (line \ref{line:oracle}). We then check if the selected edge $e^{*}$ forms (or could form) a valid tour with the elements in $\mathcal{S}$ (i.e., if $\mathcal{S} \cup \{e^{*}\} \in \mathcal{I}$) (lines \ref{line:check_start} - \ref{line:check_end}). Here, we first validate the degree constraint for each edge in $\mathcal{S} \cup \{e\}$, and then use the depth-first search (DFS) algorithm to iterate through the selected edges to check for subtours. %\footnote{A Hamiltonian cycle does not allow the existence of any subtour.}.
    If the new edge does not break the above constraints, then we add the edge in $\mathcal{S}$ and update $D$ and $\hat{H}_{cur}$ (lines \ref{line:add_edge_start} - \ref{line:add_edge_end}). Finally, we remove $e^{*}$ from $\mathcal{E}$ in line \ref{line:remove_e}.\newline 
    %\item
    \noindent \textbf{(iii) Selecting best tour set ($\mathcal{S}^{G}, \tau^{G}$)} (lines \ref{line:best_tour_start} - \ref{line:best_tour_end}): For every tour we store the value of the auxiliary function $\hat{H}$ in $\hat{H}_{\text{cur}}$, and compare it to the best value $\hat{H}_{\text{max}}$. We  store the pair $(\mathcal{S}, \tau)$ whenever $\hat{H}_{\text{cur}}> \hat{H}_{\text{max}}$, and update $\hat{H}_{\text{max}}$. 


Line 21 shows the condition of exiting the loop. As $H(\mathcal{S}, \tau)$ is concave in $\tau$, and we start from a non-negative value (as seen in Fig. \ref{fig:H_vs_tau}), it is certain that if $H(\mathcal{S}, \tau)$ becomes negative, it will continue to further decrease. This improves the runtime of \texttt{RAGA}.

\noindent \textbf{Designing the oracle function $\mathbb{O}$}: We use a sampling based oracle function to approximate $H(\mathcal{S}, \tau)$ as $\hat{H}(\mathcal{S}, \tau)$. In  \cite{ohsaka2017portfolio}, it is  proved that if the number of samples $n_{s} = O(\frac{\Gamma^{2}}{\epsilon^{2}}\log\frac{1}{\delta})$, $\delta, \epsilon \in (0,1)$, the approximation for the value of CVaR (or equivalently, the auxiliary function $\hat{H}(\mathcal{S}, \tau)$) gives an error less than $\epsilon$ with a probability of at least $1-\delta$.

\begin{algorithm}
\SetAlgoLined
\nonl \textbf{Input}: ~$G(\mathcal{V,E})$;  $\alpha \in (0,1]$; $\beta \in [0,1]$; $\Gamma \in \mathbb{R}^+$ on $\tau$; $\gamma \in (0, \Gamma]$; Oracle function $\mathbb{O}$.\\%that approximates $H(\mathcal{S}, \tau)$ as $\hat{H}(\mathcal{S}, \tau)$. \\
\nonl \textbf{Output}:  Hamiltonian tour $S^{G}$ and its respective $\tau^{G}$.\\
\For {i = \{0, 1, 2, . . ., $\ceil*{\frac{\Gamma}{\gamma}}$\}}{\label{line:for_start}
  $\mathcal{S} = \emptyset$; $D = \mathbf{0}_{1 \times |\mathcal{V}|}$; \label{line:init} $\hat{H}_{\text{max}} = 0$; $\hat{H}_{\text{cur}} = 0$, $\tau_{i} = i\,\gamma$ \\ \label{line:init_tau}
  \While {\label{line:while_start} $\mathcal{E} \neq \emptyset$ \textbf{and} $\mathcal{|S|} \leq |\mathcal{V}|$} {
    $e^\star = \text{argmax}_{{\forall e \in \mathcal{E} \setminus \mathcal{S}}} \; \hat{H}(\mathcal{S} \cup \{e\}, \tau_{i}) - \hat{H}(\mathcal{S}, \tau_{i})$\label{line:oracle}  \\ %\text{argmax}_{\forall e \in \mathcal{E} \setminus \mathcal{S}}
    $(u, v) \leftarrow \mathcal{V}(e^\star)$, $\text{flag} = \texttt{False}$\\
    \If {$D[u]<2$ \textbf{and} $D[v]<2$}{\label{line:check_start}
        check subtour existence in $\mathcal{S}\cup \{e^{\star}\}$ by running DFS\label{line:DFS}\\
        {\bf if} {\textit{no subtour present}}{~\bf then~}{ $\text{flag} = \texttt{True}$        }
    }\label{line:check_end}
    \If {$\text{flag} == \texttt{True}$}{\label{line:add_edge_start}
        $\mathcal{S} \leftarrow \mathcal{S} \cup \{e^\star\}$ \label{line:update}; $D[u] += 1$; $D[v] += 1$\\
        $\hat{H}_{\text{cur}} = \hat{H}(\mathcal{S} \cup \{e^\star\}, \tau_{i})$
   } \label{line:add_edge_end}
   $\mathcal{E} \leftarrow \mathcal{E} \setminus \{e^\star\}$ \label{line:remove_e}
  }\label{line:while_end}
  \If {$\hat{H}_{\text{cur}} \geq \hat{H}_{\text{max}}$}{\label{line:best_tour_start}
    $\hat{H}_{\text{max}} = \hat{H}_{\text{cur}}$; $(\mathcal{S}^{G}, \tau^{G})  = (\mathcal{S}, \tau_{i})$
  }\label{line:best_tour_end}
  {\bf if} {\it $\hat{H}_{\text{cur}} < 0$}~{\bf then break}\\
} \label{line:for_end}
 \caption{Risk-aware greedy algorithm (\texttt{RAGA})} \label{alg:riskg}
\end{algorithm}





\subsection{Performance Analysis}

\begin{theorem}
Let $\mathcal{S}^{G}$ and $\tau^G$ be the tour and the searching scalar selected by \texttt{RAGA} and let $\mathcal{S}^{\star}$ and $\tau^{\star}$ be the tour and the searching scalar selected the optimal solution. Then,
\begin{equation}
    H(\mathcal{S}^{G}, \tau^G)  \geq \frac{1}{2+\mathit{k}}(H(\mathcal{S}^{\star}, \tau^\star)-\gamma) + \frac{1+\mathit{k}}{2+\mathit{k}}\Gamma(1 - \frac{1}{\alpha}) - \epsilon
        \label{eqn:appro_bound}
\end{equation}
with a probability of at least $1-\delta$, when the number of samples $n_{s} = O(\frac{\Gamma^{2}}{\epsilon^{2}}\log\frac{1}{\delta}), \; \delta, \epsilon \in (0,1)$. $k$ is the curvature of $H(\mathcal{S}, \tau)$ with respect to $\mathcal{S}$.
\label{thm:approximation}
\end{theorem}

%\begin{proof}
\proof Note that $H(\mathcal{S}, \tau)$ is monotone increasing, submodular, but not normalized (Lemma \ref{lemma:properties}).  \cite[Theorem 6.1]{conforti1984submodular} and \cite[Theorem 2.10]{jawaid2013maximum} have shown that for a normalized submodular increasing function, the greedy algorithm gives an approximation of $\frac{1}{2+\mathit{k}}$ for maximizing it. Following this result, normalizing $H(\mathcal{S}, \tau)$ by $H(\mathcal{S}, \tau)-H(\emptyset, \tau)$, we get:
\begin{equation}
    \frac{H(\mathcal{S}^{G}, \tau) - H(\emptyset, \tau)}{H(\mathcal{S}^{\star}, \tau) - H(\emptyset, \tau)} \geq \frac{1}{2+\mathit{k}}
\end{equation}
where $H(\mathcal{S}^{\star}, \tau)$ is the optimal value of $H(\mathcal{S}, \tau)$ for any given value of $\tau$. Then following the proof of Theorem 1 in  \cite{zhou2020risk}, we have the bound approximation performance of \texttt{RAGA} in Equation~(\ref{eqn:appro_bound}).  $\hfill \Box$


\begin{theorem}
\texttt{RAGA} has a polynomial running time of $O(\lceil \frac{\Gamma}{\gamma} \rceil(|\mathcal{V}|^{3} (\mathcal{|V|}n_{p}+n_{s} + 2 \log |\mathcal{V}| + 1)))$.
\label{thm:complexity}
\end{theorem} 

%\begin{proof}
\proof First, the outer \textit{``for"} loop  (lines \ref{line:for_start}-\ref{line:for_end}) takes at most $\lceil \frac{\Gamma}{\gamma} \rceil$ time to search for $\tau$. Second, the inner \textit{``while"} loop (lines \ref{line:while_start}-\ref{line:while_end}) needs to check for edges $e \in \mathcal{E}$ to find the tour $\mathcal{S}$, thus running at most $|\mathcal{E}|$ times. 

Within the \textit{``while"} loop, \texttt{RAGA} finds the edge $e^{\star}$ with maximal marginal gain in line \ref{line:oracle}. To compute the marginal gain for an edge $e$, \texttt{RAGA} calls the oracle function $\mathbb{O}$. As it estimates $\hat{H}(\mathcal{S}, \tau_{i}), \forall e \in \mathcal{E} \setminus \mathcal{S}$, $\mathbb{O}$ is called at most $\mathcal{|E|}$ times, during one iteration of the \textit{``while"} loop in line \ref{line:while_start}. As \texttt{RAGA} needs to compute the marginal gains only when $\mathcal{S}$ is changed in line \ref{line:update}, and as $\mathcal{S}$ can have only $\mathcal{|V|}$ elements, it needs to perform a total of $|\mathcal{V}|$ recalculations. In addition, the edges need to be sorted every time a recalculation is performed, so that future calls to find the most beneficial element can be run in constant time without recomputing $\hat{H}(\mathcal{S}, \tau_{i})$.

For any edge $e$, the oracle $\mathbb{O}$ must compute the new mean reward and cost of $\mathcal{S} \cup \{e\}$. As only the distinct points in the environment are considered while calculating reward, the oracle must maintain an array of points that were observed while traveling along $\mathcal{S}$. If the maximum points observed when traveling along any edge in $\mathcal{E}$ is $n_{p}$, then the maximum number of points observed while traversing $\mathcal{S}$ would be $|\mathcal{V}|n_{p}$. Afterward, the oracle takes $n_{s}$ samples to compute $\hat{H}(\mathcal{S}, y)$. Thus the total runtime of the oracle is $\mathcal{|V|}n_{p}+n_{s}$. Therefore, the total time for computing gains and sorting would be $O(|\mathcal{V}|(|\mathcal{E}|(\mathcal{|V|}n_{p}+n_{s}) + |\mathcal{E}| \log |\mathcal{E}|))$.

Next, within the \textit{``while"} loop, \texttt{RAGA} checks if a the selected edge $e^{*}$ could form a valid tour with $\mathcal{S}$ (lines \ref{line:check_start}-\ref{line:check_end}). In particular, it ensures the degree of the two vertices of edge $e^\star$ is less than two (line \ref{line:check_start}). If both vertices have a degree less than two, it runs DFS to traverse the elements in $\mathcal{S}$ to check for subtours (line \ref{line:DFS}), which takes at most $|\mathcal{V}|$ time. As this is performed for every edge $e$ to be added to $\mathcal{S}$, in total, validating the selected edge runs in $O(|\mathcal{V}||\mathcal{E}|)$ time. 

Assuming that all other commands take constant time, \texttt{RAGA} has a runtime of $O(|\mathcal{V}|(|\mathcal{E}|(\mathcal{|V|}n_{p}+n_{s}) + |\mathcal{E}| \log |\mathcal{E}|) + |\mathcal{V}||\mathcal{E}|)$ for one iteration of the \textit{``for"} loop. Notably, for a complete graph, $|\mathcal{E}| = O(|\mathcal{V}|^{2})$. Considering that the \textit{``for"} loop has $\lceil \frac{\Gamma}{\gamma} \rceil$ iterations, the total runtime of \texttt{RAGA} becomes $O(\lceil \frac{\Gamma}{\gamma} \rceil(|\mathcal{V}|^{3} (\mathcal{|V|}n_{p}+n_{s} + 2 \log |\mathcal{V}| + 1)))$. $\hfill \Box$



\begin{table*}\tiny
\begin{tabularx}{\textwidth}{@{}l*{15}{C}c@{}}
\toprule 
% Group $\rightarrow$    & \multicolumn{4}{|@{}c@{\hskip0.25in}|}{Group 1} & \multicolumn{4}{@{}c@{\hskip0.25in}|}{Group 2}  & \multicolumn{3}{@{}c@{\hskip0.25in}}{Group 3} \\ 
% \midrule
\diagbox[width=3em]{\boldmath$\alpha$}{\boldmath$\beta$}  & \rotatebox[origin=c]{0}{\boldmath$0$}  & \rotatebox[origin=c]{0}{\boldmath$0.1$}  & \rotatebox[origin=c]{0}{\boldmath$0.2$}  & \rotatebox[origin=c]{0}{\boldmath$0.3$}  & \rotatebox[origin=c]{0}{\boldmath$0.4$}   & \rotatebox[origin=c]{0}{\boldmath$0.5$}  & \rotatebox[origin=c]{0}{\boldmath$0.6$}   & \rotatebox[origin=c]{0}{\boldmath$0.7$}  & \rotatebox[origin=c]{0}{\boldmath$0.8$}  & \rotatebox[origin=c]{0}{\boldmath$0.9$}  & \rotatebox[origin=c]{0}{1}  \\ \midrule
\boldmath$0.01$ & 122 \textbf{/} 145 & 121 \textbf{/} 144 & 124 \textbf{/} 141 & 126 \textbf{/} 134 & 129 \textbf{/} 136 & 127 \textbf{/} 136 & 132 \textbf{/} 138 & 127 \textbf{/} 133 & 130 \textbf{/} 131 & 132 \textbf{/} 138 & 137 \textbf{/} 135  \\
\boldmath$0.1$ & 121 \textbf{/} 149 & 122 \textbf{/} 148 & 121 \textbf{/} 149 & 125 \textbf{/} 146 & 121 \textbf{/} 145 & 136 \textbf{/} 132 & 136 \textbf{/} 137 & 135 \textbf{/} 136 & 135 \textbf{/} 133 & 130 \textbf{/} 131 & 134 \textbf{/} 131 \\ 
\boldmath$0.2$ & 124 \textbf{/} 144 & 121 \textbf{/} 143 & 124 \textbf{/} 140 & 124 \textbf{/} 147 & 134 \textbf{/} 139 & 137 \textbf{/} 139 & 144 \textbf{/} 134 & 129 \textbf{/} 138 & 138 \textbf{/} 138 & 138 \textbf{/} 130 & 134 \textbf{/} 133 \\ 
\boldmath$0.3$ & 138 \textbf{/} 137 & 127 \textbf{/} 142 & 133 \textbf{/} 133 & 135 \textbf{/} 136 & 138 \textbf{/} 138 & 138 \textbf{/} 140 & 131 \textbf{/} 144 & 140 \textbf{/} 138 & 123 \textbf{/} 144 & 127 \textbf{/} 150 & 126 \textbf{/} 141 \\
\boldmath$0.4$ & 133 \textbf{/} 138 & 142 \textbf{/} 134 & 136 \textbf{/} 135 & 129 \textbf{/} 137 & 136 \textbf{/} 139 & 138 \textbf{/} 140 & 130 \textbf{/} 141 & 139 \textbf{/} 136 & 128 \textbf{/} 147 & 127 \textbf{/} 148 & 126 \textbf{/} 147 \\ 
\boldmath$0.5$ & 141 \textbf{/} 135 & 138 \textbf{/} 135 & 144 \textbf{/} 133 & 141 \textbf{/} 138 & 142 \textbf{/} 137 & 136 \textbf{/} 139 & 138 \textbf{/} 139 & 127 \textbf{/} 148 & 138 \textbf{/} 140 & 125 \textbf{/} 147 & 129 \textbf{/} 143 \\ 
\boldmath$0.6$ & 138 \textbf{/} 131 & 141 \textbf{/} 134 & 141 \textbf{/} 134 & 142 \textbf{/} 132 & 142 \textbf{/} 137 & 134 \textbf{/} 142 & 129 \textbf{/} 142 & 134 \textbf{/} 141 & 130 \textbf{/} 144 & 124 \textbf{/} 146 & 130 \textbf{/} 146 \\
\boldmath$0.7$ & 143 \textbf{/} 133 & 138 \textbf{/} 141 & 138 \textbf{/} 138 & 139 \textbf{/} 138 & 139 \textbf{/} 138 & 137 \textbf{/} 138 & 134 \textbf{/} 141 & 131 \textbf{/} 143 & 136 \textbf{/} 140 & 129 \textbf{/} 146 & 129 \textbf{/} 147 \\ 
\boldmath$0.8$ & 143 \textbf{/} 135 & 138 \textbf{/} 137 & 141 \textbf{/} 137 & 144 \textbf{/} 133 & 142 \textbf{/} 137 & 142 \textbf{/} 137 & 141 \textbf{/} 138 & 143 \textbf{/} 135 & 129 \textbf{/} 146 & 122 \textbf{/} 148 & 126 \textbf{/} 147 \\ 
\boldmath$0.9$ & 144 \textbf{/} 133 & 139 \textbf{/} 139 & 142 \textbf{/} 135 & 144 \textbf{/} 133 & 142 \textbf{/} 137 & 140 \textbf{/} 139 & 143 \textbf{/} 136 & 128 \textbf{/} 148 & 131 \textbf{/} 146 & 121 \textbf{/} 149 & 122 \textbf{/} 150 \\
\boldmath$1$ & 143 \textbf{/} 132 & 144 \textbf{/} 132 & 144 \textbf{/} 132 & 145 \textbf{/} 134 & 145 \textbf{/} 134 & 137 \textbf{/} 137 & 134 \textbf{/} 141 & 135 \textbf{/} 139 & 121 \textbf{/} 149 & 121 \textbf{/} 149 & 128 \textbf{/} 147 \\
\bottomrule
\end{tabularx}
 \caption{\label{tab:reward_vs_cost} Variations of $f_{r}(\mathcal{S}, y)/f_{c}(\mathcal{S}, y)$ with $\alpha$ and $\beta$.}
\end{table*}



==> intro_new1.tex <==
\section{Introduction}
%\pb {The role of CVaR is missing and the motivation is missing}
Determining an optimal tour to visit all the locations in a given set while minimizing/maximizing a metric is the classical Travelling Salesperson Problem (TSP) that finds applications in robotics, logistics, etc. However, there are several applications where the environment is dynamic and uncertain, as a result of which classical approaches to solving the TSP are insufficient.
Examples include determining routes to visit active (temporal variability) volcanic regions as shown in Fig. \ref{fig:Hawaii}. %; determining routes for a logistic delivery vehicle in dense urban regions with uncertain traffic, etc.
 In such scenarios, the risk due to uncertainty in the travel times and/or the rewards collected along the path needs to be considered while determining the tour.

Several approaches to stochastic TSP have been presented in the literature.  In \cite{perboli2017progressive}, a two-step process to convert the TSP to a multi-integer linear programming problem and then introduce a meta-heuristic based on the probabilistic hedging method proposed in \cite{rockafellar1991scenarios} is carried out. Paulin \cite{paulin2014convex} uses an extension of Stein's method for exchangeable pairs to approach the stochastic salesperson problem. In \cite{maity2015modified,maity2016imprecise,mukherjee2019constrained}, a genetic algorithm is used  to consider uncertainty in TSP. In \cite{itani2007stochastic,adler2016stochastic},  approximation algorithms are developed for the stochastic TSP with Dubin's vehicle motion constraints. %visiting all the points, with cost minimization being the main objective. In \cite{adler2016stochastic}, again an approximation algorithm is presented to minimize the time taken to visit the targets that are appearing stochastically in the environment.
 In all the above articles, the risk is not considered directly. 

We argue that a different approach is necessary in many risk-sensitive applications. Specifically, instead of optimizing the expected cost, optimizing a risk-sensitive measure may be more appropriate. In this paper, we  present a risk-aware TSP formulation. To do so, we develop an approximation to the stochastic TSP with {the optimization objective} represented as a submodular function. The resulting algorithm takes  a risk tolerance parameter $\alpha$ as input and produces a tour that maximizes the expected behavior in the worst $\alpha$ percentile cases. Thus, the user can choose tours ranging from risk-neutral ($\alpha = 1$) to very conservative ($\alpha\approx 0$).
\begin{figure*}
\begin{multicols}{5}
    \includegraphics[width=3cm,height=3.5cm]{figs/map_filled.eps}\subcaption{}\label{fig:map_Hawaii}\par
    \includegraphics[width=3cm,height=3.5cm]{figs/key_points.eps}\subcaption{}\label{fig:key_points}\par
    \includegraphics[width=3cm,height=3.5cm]{figs/high_cost_high_reward.eps}\subcaption{}\label{fig:high_cost_high_reward}\par
        \includegraphics[width=3cm,height=3.5cm]{figs/low_cost_low_reward.eps}\subcaption{}\label{fig:low_cost_low_reward}\par 
        \includegraphics[clip,trim=20mm 8mm 20mm 15mm, width=3cm,height=3.5cm]{figs/info_map.png}\subcaption{}\label{fig:info_map}\par 
\end{multicols}\vspace{-0.4cm}
\caption{An example of risk-aware tour selection for volcano monitoring in an island. (a) The areas of active volcanoes (red regions) (b) Key sites of surveillance surrounding the volcanic sites (c) Tour with high cost and high reward (d) Tour with low cost and low reward (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
\end{figure*}

%\begin{figure*}[t]
%\begin{multicols}{4}
%    \includegraphics[width=3cm,height=4cm]{figs/map_filled.eps}\subcaption{}\label{fig:map_Hawaii}\par
%    \includegraphics[width=3cm,height=4cm]{figs/key_points.eps}\subcaption{}\label{fig:key_points}\par
%    \includegraphics[width=3cm,height=4cm]{figs/high_cost_high_reward.eps}\subcaption{}\par
%        \includegraphics[width=3cm,height=4cm]{figs/low_cost_low_reward.eps}\subcaption{}\label{fig:low_cost_low_reward}\par 
%        \includegraphics[width=3cm,height=4cm]{figs/info_map.png}\subcaption{Tour with low cost and low reward}\label{fig:info_map}\par 
%\end{multicols}
%\caption{An example of risk-aware tour selection for volcano monitoring in an island. (a). An island with the locations of active volcanoes (red regions) (b) Key sites of surveillance surrounding the volcanic sites (c) Tour with high cost and high reward}\label{fig:high_cost_high_reward (d) Tour with low cost and low reward (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
%\end{figure*}
%\begin{figure*}[t]
%\begin{multicols}{4}
%    \includegraphics[width=3cm,height=4cm]{figs/map_filled.eps}\subcaption{An island with the locations of active volcanoes (red regions)}\label{fig:map_Hawaii}\par
%    \includegraphics[width=3cm,height=4cm]{figs/key_points.eps}\subcaption{Key sites of surveillance surrounding the volcanic sites}\label{fig:key_points}\par
%    \includegraphics[width=3cm,height=4cm]{figs/high_cost_high_reward.eps}\subcaption{Tour with high cost and high reward}\label{fig:high_cost_high_reward}\par
%        \includegraphics[width=3cm,height=4cm]{figs/low_cost_low_reward.eps}\subcaption{Tour with low cost and low reward}\label{fig:low_cost_low_reward}\par 
%        \includegraphics[width=3cm,height=4cm]{figs/info_map.png}\subcaption{Tour with low cost and low reward}\label{fig:info_map}\par 
%\end{multicols}
%\caption{An example of risk-aware tour selection for volcano monitoring in an island. A low-risk, low-reward monitoring tour avoids the more interesting region in the middle which the high-risk, high-reward tour covers. (e) Map $M$ shows the information distribution in the environment $E$.}\label{fig:Hawaii} \vspace{-0.75cm}
%\end{figure*}
An important property of submodular functions are their diminishing marginal values. The use of submodular functions is wide-spread: from information gathering \cite{krause2011submodularity} and image segmentation \cite{boykov2001interactive} to document summarization \cite{lin2011class}. Rockafellar and Uryasev \cite{rockafellar2000optimization} introduces a relationship between a  submodular function and the Conditional-Value-at-Risk (CVaR). CVaR is a risk metric that is commonly employed in stochastic optimization in finance and stock portfolio optimization.
%They then propose an auxiliary function by which the CVaR can be maximized. 
Another popular measure of risk is the Value-at-Risk (VaR) \cite{morgan1997creditmetrics}, which is commonly used to formulate the chance-constrained optimization problems.
In \cite{yang2017algorithm}, and \cite{yang2018algorithm}, the authors study the chance-constrained optimization problem while also considering risk in the multi-robot assignment problems. In a comparison between the VaR and CVaR, Majumdar and Pavone \cite{majumdar2020should} propose that the CVaR is a better measure of risk for robotics, especially when the risk can cause a huge loss. In \cite{zhou2018approximation} and \cite{zhou2020risk}, a greedy algorithm for maximizing the CVaR is proposed.  

Building on the work by \cite{zhou2018approximation,zhou2020risk}, in this paper, %we leverage this prior work on choosing an unordered set to develop the first risk-aware optimization for choosing an ordered tour. {Our major contribution is the
we develop a polynomial-time algorithm for approximating a solution to the stochastic TSP. Our method differs from the previous approaches due to the presence of uncertainty in the tour cost, making traditional path-planning algorithms fail. The framework presented in \cite{zhou2018approximation,zhou2020risk} is effective only for one-stage planning (selecting a path amongst a set of candidate paths). In this paper, we present a multi-stage planner that finds a route taking the stochastic aspect into account. To achieve this, we propose an objective function that balances  risk and reward for a tour and prove that this function is submodular. %  whereas the algorithm developed in this paper finds a balance between two opposing functions formed from the rewards and costs. Our algorithm plans an entire TSP tour, which is fundamentally more challenging than selecting a path amongst a set of candidate paths for the vehicle assignment in \cite{zhou2018approximation,zhou2020risk
%We can say 15-16 were not designed for finding tours but just selecting from amongst a set of candidate paths. Here, we are *planning* for a path so the algorithm needs to take that into account. We can also say that another novel contribution is this function that balancesand showing that it is submodular.
 The method in \cite{jawaid2013maximum} addresses the deterministic TSP with a reward-cost trade-off, while our work is focused  on a stochastic version where the uncertainty in reward and cost is considered. The algorithm from \cite{jawaid2013maximum} can be viewed as a special case of our algorithm, with $\alpha=1$ and the subsequent risk ignored.
%We determine a single solution set to maximize the CVaR using a monotone submodular function \cite{zhou2018approximation}. The optimization problem is then framed over a matroid constrained system.


\noindent \textbf{Contributions}:  The main contributions of this paper are:
\begin{itemize}[leftmargin=*]%Risk-Aware Multi Objective%
    \item \textcolor{black}{We present a risk-aware TSP with a stochastic objective that balances risk and reward for planning a TSP tour (Problem~\ref{prob:risk-tsp}). 
    \item We show the objective is submodular (Lemma~\ref{lemma:sub and monotone}) and }propose a greedy algorithm (\texttt{RAGA}) to find tours that maximize the CVaR of a stochastic objective (Algorithm~\ref{alg:riskg}).
    \item We prove that the solution obtained by \texttt{RAGA} is within a constant approximation factor of the optimal and an additive term proportional to the optimal solution (Theorem~\ref{thm:approximation}) and prove that \texttt{RAGA} has a polynomial run-time (Theorem~\ref{thm:complexity}). 
    \item We evaluate the performance of the algorithm through extensive simulations (Section~\ref{sec: results}).
\end{itemize}

% \indent \textbf{Organization}: The rest of the paper is organized as follows. In Sec. \ref{sec: prelim}, the necessary background materials on  sets, function properties, VaR, and CVaR is given. In Sec. \ref{sec: prob_form}, we describe risk-aware  TSP and the multi-objective optimization problem. Subsequently, we present our main algorithm \texttt{RAGA} and then derive its performance in Sec. \ref{sec: algo_&_analysis}. In Sec. \ref{sec: results}, we show simulation results of \texttt{RAGA}. Finally, in Sec. \ref{sec: conc}, we conclude and discuss future work.

==> intro_old.tex <==
\section{Introduction}

%\pb {The role of CVaR is missing and the motivation is missing}

The maximum weight Hamiltonian cycle (max-TSP), is a well-researched NP-hard problem, which can also be formed as a minimization problem, where tour cost is minimized. Because of its computation intensity, there have been no known polynomial-time solutions but several approximation algorithms. A common method of approaching the problem is using graph theory concepts to find a minimum spanning tree. In \cite{christofides1976worst}, Christofides develops an algorithm to search for the shortest spanning subtree with minimum cost, which has a $\frac{3}{2}$ approximation. In \cite{fisher1979analysis}, the authors give approximation bounds on undirected graphs with non-negative weights. They go on to prove that the greedy, best neighbor and 2-interchange heuristics give a $\frac{1}{2}$ approximation, while the perfect 2-matching gives a $\frac{2}{3}$ approximation. The authors of \cite{jawaid2013maximum}, develop two approximation algorithms on a submodular cost function with an approximation factor of $\frac{1}{2+k}$ and $\max\{\frac{2}{3(2+k)}, \frac{2(1-k)}{3})\}$, where $k$ is the curvature of the function.

Another popular idea is using Linear Programming techniques to find a solution, given certain bounds on the variables. Bellman \cite{bellman1962dynamic} introduces a simple method for formulating the TSP in dynamic programming terms. Similarly, the authors in \cite{gavish1978travelling} use the Lagrangian Relaxation and sub-gradient optimization to approach the Inter Programming TSP.

Recently, there has been a rise in evolutionary algorithms, meta-agents, and learning methods to tackle the TSP. In \cite{akhand2020discrete}, the authors use a meta-agent to find near-optimal paths. In \cite{joshi2019efficient}, the authors create a Graph Convolutional Neural Network to solve the TSP approximately. Another idea was to build a policy network that improves an initial solution by iteratively performing a neighborhood search \cite{wulearning}. 

The problem complexity increases when the uncertainty in tour quality is also considered. In \cite{perboli2017progressive}, the authors use a two-step process to convert the TSP to a multi-integer linear programming problem and then introduce a meta-heuristic based on the probabilistic hedging method proposed in \cite{rockafellar1991scenarios}. Paulin \cite{paulin2014convex} uses an extension of Stein's method for exchangeable pairs to approach the stochastic salesman problem. In \cite{maity2015modified}, \cite{maity2016imprecise} and \cite{mukherjee2019constrained}, the authors develop a genetic algorithm to approach the uncertainty in TSP. In this paper, we take a graph-based approach to generate an approximation to the stochastic TSP by using a submodular function. 
%\lz{it would be better to replace this paragraph by the work on TSP with uncertainty/stochastic tsp, then it can naturally transition to the next paragraph} \rb{addressed} \lz{exchange these 2 for a better organisation}


\begin{figure*}[t]
\begin{multicols}{4}
    \includegraphics[width=\linewidth]{figs/map_filled.eps}\subcaption{A map of Hawaii, with the locations of active volcanoes highlighted in red}\label{fig:map_Hawaii}\par
    \includegraphics[width=\linewidth]{figs/key_points.eps}\subcaption{Key points of surveillance surrounding the volcanic sites}\label{fig:key_points}\par
    \includegraphics[width=\linewidth]{figs/low_cost_low_reward.eps}\subcaption{Path with low cost and low reward}\label{fig:low_cost_low_reward}\par 
    \includegraphics[width=\linewidth]{figs/high_cost_high_reward.eps}\subcaption{Path with high cost and high reward}\label{fig:high_cost_high_reward}\par
\end{multicols}
\caption{An example of site placement and risk-aware path selection for volcano surveillance in Hawaii.}\label{fig:Hawaii} 
%\lz{fig1 and 2 together}
\end{figure*}

An important property of submodular functions is its diminishing marginal values. The use of submodular functions is wide-spread: from information gathering \cite{krause2011submodularity} and image segmentation \cite{boykov2001interactive} to document summarization \cite{lin2011class}. Rockafellar and Uryasev introduce a relationship between a monotone increasing, normalized, submodular function, and the Conditional-Value-at-Risk (CVaR) \cite{rockafellar2000optimization}, and propose an auxiliary function by which the CVaR can be maximized. Another measure of risk is the Value-at-Risk (VaR)\cite{morgan1997creditmetrics}, which is commonly used to formulate the chance-constrained optimization problems. In \cite{yang2017algorithm}, and \cite{yang2018algorithm}, the authors study the chance-constrained optimization problem while also considering risk in multi-robot assignment, and then extend it to a knapsack formulation. In a comparison between the VaR and CVaR, Majumdar and Pavone argue that the CVaR is a better measure of risk for robotics based on six axioms \cite{majumdar2020should}. Finally, in \cite{zhou2018approximation} and \cite{zhou2020risk}, the authors demonstrate a greedy algorithm for maximizing the CVaR.  

\indent \textbf{Contributions}: We focus on selecting a single solution set, similar to \cite{zhou2018approximation}, to maximize the CVaR using a monotone submodular function. The optimization problem is then framed over a matroid constrained system. Our contributions are as follows:

\begin{itemize}%Risk-Aware Multi Objective%
    \item We propose the Risk Aware Greedy Algorithm (\texttt{RAGA}) to select tours for the Travelling Salesman Problem that maximize the value of CVaR.
    \item We then prove that the solution found is within a constant approximation factor of the optimal set added with an additive term proportional to the optimal solution. Next, we prove that the proposed algorithm has a polynomial runtime. 
    \item We finally test the performance of the algorithm through simulations.
\end{itemize}

\indent \textbf{Organization}: The rest of the paper is organized as follows. In Sec. \ref{sec: prelim}, we discuss the necessary background material on graphs, sets, and function properties. We then formally define the concepts of VaR and CVaR. Next, in Sec. \ref{sec: prob_form}, we describe the setting of the TSP and the multi-objective optimization. Subsequently, we present the Risk Aware Greedy algorithm and then derive its performance in Sec. \ref{sec: algo_&_analysis}. In Sec. \ref{sec: results}, we show simulation results of the algorithm. Finally, in Sec. \ref{sec: conc}, we conclude and discuss the work remaining.

% \indent \textbf{Related work.}\\

%  \lz{\begin{itemize}
%   \item introduce our risk-aware TSP (refer to my WAFR paper.)
%     \item Related work, part 1: TSP, stochastic TSP using expectation, mean-variance measure, chance constraint etc. (need some search)
%     \item Related work, part 2: VaR and CVaR for robot planning. (refer to my WAFR paper.)
%     \item our contributions, 1: formulate risk-aware TSP; 2:approximation bound and polynomial running time; 3: simulation results. (Refer to my IROS paper) 
%  \end{itemize}}

==> prelim.tex <==
\section{Preliminaries}\label{sec: prelim}
We first introduce the conventions and notations used in this paper. Calligraphic capital letters denote sets (e.g. $\mathcal{A}$). $2^{\mathcal{A}}$ denotes the power set of $\mathcal{A}$ and $|\mathcal{A}|$ represents its cardinality. Given a set $\mathcal{B}$, $\mathcal{A \setminus B}$ denotes set difference. Let $x$ be a random variable, then $\mathbb{E}[x]$ represents the expectation of the random variable $x$, and $\mathbb{P[\cdot]}$ denotes its probability. 

\subsection{Set and Function Properties}
Optimization problems generally work over a set system $(\mathcal{X, Y})$ where $\mathcal{X}$ is the base set and $\mathcal{Y} \subseteq 2^{\mathcal{X}}$. A reward/cost function $f : \mathcal{Y} \rightarrow \mathbb{R}$ is then either maximized or minimized. 

\begin{definition}
\label{def:inc}
(Monotonically Increasing):  A set function $f : \mathcal{Y} \rightarrow \mathbb{R}$ is said to be monotonically increasing if and only if for any set $\mathcal{S'} \subseteq \mathcal{S} \in 2^{\mathcal{X}}, ~f(\mathcal{S'}) < f(\mathcal{S})$.
\end{definition}
\begin{definition}
\label{def:sub}
(Submodularity): A function $f:2^{\mathcal{X}} \rightarrow \mathbb{R}$ is submodular if and only if,
$f(\mathcal{S}) + f(\mathcal{T}) \geq f(\mathcal{S} \cup \mathcal{T}) + f(\mathcal{S} \cap \mathcal{T}), ~\forall \mathcal{S},~\mathcal{T}~\in~2^{\mathcal{X}}$.

\end{definition}
\begin{definition}
(Matroid): An independence set system $\mathcal{(X,Y)}$ is called a matroid if for any sets $\mathcal{S, P} \in 2^{\mathcal{X}}$ and $|\mathcal{P}| \leq |\mathcal{S}|$, it must hold that there exists an element $s \in \mathcal{S} \setminus \mathcal{P}$ such that $\mathcal{P} \cup \{s\} \in \mathcal{Y}$.
\end{definition}

\begin{definition}
(Curvature): Curvature is used as a measure of the degree of submodularity of a function $f$. Consider the matroid pair $(\mathcal{X, Y})$, and a function $f: 2^{\mathcal{X}} \rightarrow \mathbb{R}$, such that for any element $s \in \mathcal{X}, f(\{s\}) \neq 0$. The curvature $k,0 \leq k \leq 1$ is then defined as:
\begin{equation}\small
    k = 1 - \min_{s \in \mathcal{S}, \mathcal{S} \in \mathcal{Y}} \: \frac{f(\mathcal{S}) - f(\mathcal{S}\setminus \{s\})}{f(\{s\})}.
\end{equation}
\end{definition}\vspace{-0.3cm}

\subsection{Travelling Salesperson Problem}

\begin{definition}
(TSP): Given a complete graph $G(\mathcal{V, E})$, the objective of the TSP is to find a minimum cost (maximum reward) Hamiltonian cycle. 
\end{definition}
In this paper, we consider the symmetric undirected TSP, where each edge has a reward and cost associated with it. \vspace{-0.3cm}




\subsection{Measure of Risk}
Let $f(\mathcal{S}, y)$ denote a utility function with solution set $\mathcal{S}$ and noise $y$. As a result of $y$, the value of $f(\mathcal{S},y)$ is a random variable for every $\mathcal{S}$. 
\begin{definition}
    (Value at Risk): The Value at Risk (VaR) is defined as:
\begin{equation}
    \emph{VaR}_{\alpha}(\mathcal{S}) = \min_{\tau \in \mathbb{R}} \; \{\mathbb{P}[f(\mathcal{S}, y) \leq \tau] \geq \alpha \}, \; \alpha \in (0,1],
\end{equation}
\textcolor{black}{where $\alpha$ is the user-defined risk-level. A higher value of $\alpha$ corresponds to the choice of a higher risk level}.
\end{definition}

\begin{definition}
    (Conditional Value at Risk): The Conditional-Value-at-Risk (CVaR) is defined as
\begin{equation}
    \emph{CVaR}_{\alpha}(\mathcal{S}) = \mathbb{E}_{y} [f(\mathcal{S},y) \:|\: f(\mathcal{S},y) \leq \emph{VaR}_{\alpha}(\mathcal{S})].
\end{equation}
Maximizing the value of $\text{CVaR}_{\alpha}(\mathcal{S})$ is equivalent to maximizing the auxiliary function $H(\mathcal{S}, \tau)$ (Theorem 2, \cite{rockafellar2000optimization}):
\begin{equation}
    H(\mathcal{S}, \tau) = \tau - \frac{1}{\alpha}\mathbb{E}_y[\: (\tau - f(\mathcal{S}, y))^{+} \:],
\end{equation}
where $[t]^{+} = t, ~\forall t \geq 0$ and $0$ when $t < 0$.
\end{definition}



\begin{lemma}
\label{lemma:properties}
\textup{(Lemma 1, \cite{zhou2018approximation})} If $f(\mathcal{S},y)$ is monotone increasing, submodular and normalized in set $\mathcal{S}$ for any realization of $y$, then the auxiliary function $H(\mathcal{S}, \tau)$ is monotone increasing and submodular but not necessarily normalized \footnote{\textcolor{black}{The function $f(\mathcal{S}, y)$ is normalized in $\mathcal{S}$ if and only if $f(\emptyset, y) = 0$.}} in set $\mathcal{S}$ for any given $\tau$.
\end{lemma} 

\begin{lemma}
\textup{(Lemma 2, \cite{zhou2018approximation})} The auxiliary function $H(\mathcal{S}, \tau)$ is concave in $\tau, \forall\: \mathcal{S}$.
\end{lemma}



==> probFormulation.tex <==
\section{Problem Formulation} \label{sec: prob_form}
In this section, we first discuss a risk-aware TSP and then formulate the problem as a  stochastic optimization problem by using CVaR.

\subsection{Risk-Aware TSP}
In order to motivate our formulation, consider the scenario of monitoring active volcanoes using a robot (say aerial robot) on an island as shown in Fig. \ref{fig:map_Hawaii}, where the red-colored patches represent active volcanic regions.  The important sites ($\mathcal{V}$) that the robot needs to visit are shown in Fig. \ref{fig:key_points}. \textcolor{black}{These sites are strategic positions from which it is possible to observe the volcanic situation from a safe distance.} The robot travels between these monitoring sites and receives a reward based on the information gathered while traversing this tour.  While traveling directly above the volcano, the robot faces a higher chance of failure (due to volcanic activity) but can gather more information (a higher reward) and a shorter path (less cost) Fig. \ref{fig:high_cost_high_reward}. On the other hand, while traveling around the volcano, the robot has a lower risk but must travel a longer distance (more cost) while also receiving a lower reward Fig. \ref{fig:low_cost_low_reward} .  Our objective is to find a suitable tour for a single robot while considering the risk threshold and the trade-off between path cost and reward required. 

The monitoring task is modeled as a risk-aware TSP on a graph $G(\mathcal{V}, \mathcal{E})$ of an environment ${E}$ with $|\mathcal{V}|$ sites of interest and  $\mathcal{E}$ represents the set of edges connecting the vertices. A representative information density map ${M}$ of the environment ${E}$ is shown in Fig. \ref{fig:info_map}. The robot has sensors with a sensing range $R$. As it travels along the tour, the robot receives a reward based on the amount of information it collects and a penalty proportional to the tour's cost. We assume that both the reward and cost are random variables, with the reward being positive, and the cost of every edge having an upper-bound of $C$. {We use $r(\mathcal{S}, y_{r})$ and $c(\mathcal{S}, y_{c})$ to denote the reward and cost for the edge set  $\mathcal{S}$, where $r(\mathcal{S})$ and $c(\mathcal{S})$ are the sum of rewards of all points observed and the costs incurred when travelling along the edges in set $\mathcal{S}$ respectively, and  $y_{r}$ and $y_{c}$ are the respective noises induced.}


As we want to minimize cost and maximize reward simultaneously, our utility function $f(\mathcal{S},y)$ is a combination of these two terms, with a weighting factor deciding the priority of cost over the reward. We define $f(\mathcal{S},y)$ as
\begin{equation}
    f(\mathcal{S}, y) = (1-\beta)\:r(\mathcal{S}, y_{r}) +  \beta\:(|\mathcal{S}|C-c(\mathcal{S}, y_{c})),
\end{equation}
where $\beta \in [0,1]$ is the weighting parameter. When $\beta = 0$, we ignore the cost incurred and consider the rewards received only. When $\beta = 1$, we ignore the rewards and are wary of only the cost penalized (classical TSP). Note that we directly incorporate the cost-reward trade-off into the utility function. Let us define $r(\mathcal{S}, y_{r})$ as $f_{r}(\mathcal{S}, y_{r})$ and $|\mathcal{S}|C-c(\mathcal{S}, y_{c})$ as $f_{c}(\mathcal{S}, y_{c})$. 

%\begin{figure}
%    \centering
%    \includegraphics[width=6cm, height=4cm]{figs/info_map.png}
%    \caption{Map $M$ shows the information distribution in the environment $E$.} % with the density  information.}
%    \label{fig:info_map}\vspace{-0.75cm}
%\end{figure}

\begin{lemma}
The utility function $f(\mathcal{S}, y)$ is both submodular and monotone increasing in $\mathcal{S}$.
\label{lemma:sub and monotone}
\end{lemma}

%%%%%%%%%%%%%%NEW VERSION TEXT

\proof {Let $e$ be the edge to be added to the tour, where $e \in \mathcal{E} \setminus \mathcal{S}$ and $\mathcal{S}$ is set of edges selected so far. Let us consider the two parts of $f(\mathcal{S}, y)$ separately. 
 \newline {\bf (a) {$f_{r}(\mathcal{S},y)$}}: As the rewards are sampled from a truncated Gaussian, with a lower bound of 0, they are thus always positive. Therefore, $f_{r}(\mathcal{S}, y)$ is always monotone increasing in $\mathcal{S},            f_{r}(\mathcal{S}) \leq f_{r}(\mathcal{S}\cup\{e\})$.
\newline \noindent While calculating the total reward, we add the rewards obtained from all \textit{distinct} points observed while traversing this tour. Consider the current set of edges $\mathcal{S}$ and a new edge $e$. If the new edge $e$ and the edges $\mathcal{S}$ have any overlap in the sensed regions, the total reward received from traversing $\mathcal{S}$ and $e$ successively will be less than the sum of rewards of traversing $\mathcal{S}$ and $e$ individually. Therefore,
 $ f_{r}(\mathcal{S} \cup \{e\})  \leq f_{r}(\mathcal{S}) + f_{r}(\{e\})$. Also, since $e \in \mathcal{E} \setminus \mathcal{S}$, $f_{r}(\mathcal{S} \cap \{e\}) =0$. Then we have, $
            f_{r}(\mathcal{S} \cup \{e\}) + f_{r}(\mathcal{S} \cap \{e\}) \leq f_{r}(\mathcal{S}) + f_{r}(\{e\}),$ 
        and thus $f_{r}(\mathcal{S},y)$ is submodular in $\mathcal{S}$.

\noindent{\bf(b) {$f_{c}(\mathcal{S}, y)$}}: The cost of each edge is defined as a truncated Gaussian with a upper bound of $M_{c}$. For any set of edges in $\mathcal{S}$, the sum of costs will always be less than $|\mathcal{S}|M_{c}$, which means any sample (realization) of $f_{c}(\mathcal{S}, y)$ is positive. Therefore, $f_{c}(\mathcal{S}, y)$ is always monotone increasing in $\mathcal{S}$,  $ f_{c}(\mathcal{S}) \leq f_{c}(\mathcal{S}\cup\{e\}).$ Consider again, the current set of edges $\mathcal{S}$ and the new edge $e$. The total cost of traversing $\mathcal{S}$ and $e$ is equal to the sum of costs of  traversing $\mathcal{S}$ and $e$ individually. Therefore,
$            f_{c}(\mathcal{S} \cup \{e\}) = f_{c}(\mathcal{S}) + f_{c}(\{e\}), $
        and thus $f_{c}(\mathcal{S}, y)$ is modular in $\mathcal{S}$.
\newline \noindent {\bf (c) {$f(\mathcal{S}, y)$}}: Since both $f_{r}(\mathcal{S}, y_{r})$ and $f_{c}(\mathcal{S}, y_{c})$ are monotone increasing in $\mathcal{S}$, $f(\mathcal{S}, y)$ as the summation of these two, is also monotone increasing in $\mathcal{S}$. Similarly, since $f_{r}(\mathcal{S}, y_{r})$ is submodular in $\mathcal{S}$ and $f_{c}(\mathcal{S}, y_{c})$ is modular in $\mathcal{S}$, $f(\mathcal{S}, y)$ as the summation of these two, is submodular in $\mathcal{S}$.  \hfill $\Box$ 
}

\subsection{Risk-Aware  Submodular Maximization}
Consider the set system $\mathcal{(E, I)}$, where $\mathcal{E}$ is the set of all edges in the graph $G(\mathcal{V, E})$. If $\mathcal{A}_{1}, \mathcal{A}_{2} \ldots \mathcal{A}_{n}$ each contains the edges forming $n$ Hamiltonian tours, then $\mathcal{I} := 2^{\mathcal{A}_{1}} \cup 2^{\mathcal{A}_{2}} \ldots \cup 2^{\mathcal{A}_{n}}$. We define our \textit{risk-aware  TSP} by maximizing  $\text{CVaR}_{\alpha}(\mathcal{S})$, where $\mathcal{S} \in \mathcal{I}$. We know that maximizing the $\text{CVaR}_{\alpha}(\mathcal{S})$ is equivalent to maximizing the auxiliary function ${H(\mathcal{S}, \tau)}$. Thus, we formally define the problem as:

\begin{problem} [Risk-aware  TSP]
\begin{equation}
    \max_{\mathcal{S} \in \mathcal{I}, ~\tau \in [0, \Gamma]} \tau - \frac{1}{\alpha} \mathbb{E}_y[ (\tau - f(\mathcal{S}, y))^{+}], 
\end{equation}
where $\Gamma$ is the upper bound on the value of $\tau$.
\label{prob:risk-tsp}
\end{problem}


